Contextual Bandits with Online Neural Regression

Recent works have shown a reduction from contextual bandits to online regression under a realizability assumption [Foster and Rakhlin, 2020, Foster and Krishnamurthy, 2021]. In this work, we investigate the use of neural networks for such online regression and associated Neural Contextual Bandits (NeuCBs). Using existing results for wide networks, one can readily show a ${\mathcal{O}}(\sqrt{T})$ regret for online regression with square loss, which via the reduction implies a ${\mathcal{O}}(\sqrt{K} T^{3/4})$ regret for NeuCBs. Departing from this standard approach, we first show a $\mathcal{O}(\log T)$ regret for online regression with almost convex losses that satisfy QG (Quadratic Growth) condition, a generalization of the PL (Polyak-\L ojasiewicz) condition, and that have a unique minima. Although not directly applicable to wide networks since they do not have unique minima, we show that adding a suitable small random perturbation to the network predictions surprisingly makes the loss satisfy QG with unique minima. Based on such a perturbed prediction, we show a ${\mathcal{O}}(\log T)$ regret for online regression with both squared loss and KL loss, and subsequently convert these respectively to $\tilde{\mathcal{O}}(\sqrt{KT})$ and $\tilde{\mathcal{O}}(\sqrt{KL^*} + K)$ regret for NeuCB, where $L^*$ is the loss of the best policy. Separately, we also show that existing regret bounds for NeuCBs are $\Omega(T)$ or assume i.i.d. contexts, unlike this work. Finally, our experimental results on various datasets demonstrate that our algorithms, especially the one based on KL loss, persistently outperform existing algorithms.

==> app/app_neuralCBcomp.tex <==


% %We consider the setting with $K=1$. 
% In this section we show that the regret bounds for NeuralUCB \citet{zhou2020neural} and Neural Thompson Sampling (NeuralTS) \citep{zhang2021neural} could be $\Omega(T)$ rendering them useless. We start with a brief description of the notations used in these works.
% $\bH$ is the Neural Tangent Kernel (NTK) matrix computed from all the context vectors $\x_{t,i}$, $t \in [T], i \in [K]$, and $h(\x)$ is the true reward function given a context $\x$. The cumulative reward vector is defined as $\bh = (h(\x_1),\ldots,h(\x_{TK}))^T$.

% With $\lambda$ as the regularization parameter in the loss, the effective dimension $\tilde{d}$ of the Neural Tangent Kernel $\bH$ on the contexts $\{\x_{t}\}_{t=1}^{TK}$ is defined as:
% \begin{align*}
%     \tilde{d} = \frac{\log \det(\bI+\bH/\lambda)}{\log(1+T/\lambda)}
% \end{align*}
% Further it is assumed that $\bH \succeq \lambda_0 \I$ (see Assumption 4.2 in \citep{zhou2020neural} and Assumption 3.4 in \citep{zhang2021neural}).
% \subsection{\texorpdfstring{$\Omega(T)$}{alpha} regret for NeuralUCB \citep{zhou2020neural}}
% The bound on the regret for NeuralUCB is given by (ignoring constants):
% \begin{align*}
%     \reg(T) &\leq \sqrt{T}\sqrt{\tilde{d}\log\left(1+\frac{TK}{\lambda}\right)} \left(\sqrt{\tilde{d}\log\left(1+\frac{TK}{\lambda}\right)} + \sqrt{\lambda} S\right)\\
%     &= \sqrt{T} \left(\tilde{d}\log\left(1+\frac{TK}{\lambda}\right) + S\sqrt{\tilde{d} \log\left(1+\frac{TK}{\lambda}\right)\lambda}\right) \coloneqq \bnucb(T,\lambda),
% \end{align*}
% where, $\lambda$ is the regularization constant and $S \geq \sqrt{\bh^TH^{-1}\bh}$ with $\bh = (h(\x_1),\ldots,h(\x_{TK}))^T$. We provide two $\Omega(T)$ regret bounds for NeuralUCB. The first result is an existential result in the sense that it says there exists a reward function such that the bound is $\Omega(T)$. The second result provides an $\Omega(T)$ bound for any reward function and set of context vectors as long as $\|\bh\|_2$ and the condition number of $\bH$ are $\Theta(1)$. 
% \begin{proposition}
% \label{prop:nucb_1}
%     There exists a reward vector $\bh$ such that the regret bound for NeuralUCB is lower bounded as
%     \[\emph{$\bnucb$}(\lambda,T) \geq \displaystyle\frac{1}{\sqrt{2}}\sqrt{K}T.\]
% \end{proposition}

% \begin{proof}
%     Consider the eigen-decomposition of $\bH = U \Sigma_{\bH} U^T$,
% where columns of $U \in \R^{TK \times TK}$ are the normalized eigen-vectors $\{u_i\}_{i=1}^{TK}$ of $\bH$ and $\Sigma_{\bH}$ is a diagonal matrix containing the eigenvalues $\{\lambda_{i}(\bH)\}_{i=1}^{TK}$ of $H$. Now,
% \begin{align}
% \label{eq:S_lower}
%     S &\geq \sqrt{\bh^T \bH^{-1}\bh}\nonumber \\
%     &= \sqrt{\bh^TU \Sigma_{\bH}^{-1} U^T \bh}\nonumber \\
%     &= \sqrt{\sum_{i=1}^{TK} \frac{1}{\lambda_i(\bH)} (u_i^Th)^2}\nonumber \\
%     &\geq \xi \sqrt{\sum_{i=1}^{TK} \frac{1}{\lambda_i(\bH)}},\\
%     \text{where } \xi &= \min_{i} (u_i^T \bh)^2 \nonumber
% \end{align}
% Further observe that we can rewrite the effective dimension as follows:
% \begin{align*}
%     \tilde{d} = \frac{\log \det(\bI+\bH/\lambda)}{\log(1+TK/\lambda)} = \frac{\log \left(\displaystyle\prod_{i=1}^{TK}\left(1+\frac{\lambda_{i}(\bH)}{\lambda}\right)\right)}{\log(1+TK/\lambda)}
%     = \frac{\displaystyle \sum_{i=1}^{TK} \left(1+\frac{\lambda_{i}(\bH)}{\lambda}\right)}{\log (1+{TK}/{\lambda})}\\
% \end{align*}

% Using these we can lower bound $\bnucb(T,\lambda)$ as follows:
% \begin{align*}
%     \bnucb(T,\lambda) &\geq \sqrt{T} \Bigg( \sum_{i=1}^{TK}\frac{\log \left(1+\frac{\lambda_{i}(\bH)}{\lambda}\right)}{\log\left(1+\frac{TK}{\lambda}\right)}\log\left(1+\frac{TK}{\lambda}\right) \\
%     &\qquad \qquad + \xi \sqrt{ \sum_{i=1}^{TK}\frac{\lambda}{\lambda_{i}(\bH)}\sum_{i=1}^{TK}\frac{\log(1 + \frac{\lambda_{i}(\bH)}{\lambda})}{\log\left(1+\frac{TK}{\lambda}\right)}\log\left(1+\frac{TK}{\lambda}\right)}\Bigg)\\
%     &= \sqrt{T} \left(\sum_{i=1}^{TK}{\log \left(1+\frac{\lambda_{i}(\bH)}{\lambda}\right)} + \xi \sqrt{ \sum_{i=1}^{TK}\frac{\lambda}{\lambda_{i}(\bH)}\sum_{i=1}^{TK}{\log\left(1 + \frac{\lambda_{i}(\bH)}{\lambda}\right)}}\right)\\
%     &\geq \sqrt{T} \left(\sum_{i=1}^{TK}{\log \left(1+\frac{\lambda_{i}(\bH)}{\lambda}\right)} + \xi \sqrt{ \sum_{i=1}^{TK}\frac{\lambda}{\lambda_{i}(\bH)}{\log\left(1 + \frac{\lambda_{i}(\bH)}{\lambda}\right)}}\right)\\
%     &= \sqrt{T} \left(\sum_{i=1}^{TK}{\log \left(1+\frac{1}{y_i}\right)} + \xi \sqrt{\sum_{i=1}^{TK}y_i{\log\left(1 + \frac{1}{y_i}\right)}}\right),\\
% \end{align*}
% where $y_i = \frac{\lambda}{\lambda_{i}(\bH)}$, $i \in [TK]$. Using this we can further bound $\bnucb(T,\lambda)$ as follows:
% \begin{align*}
%     \bnucb(T,\lambda) 
%     &\geq \sqrt{T} \left(\sum_{i=1}^{TK}{\log \left(1+\frac{1}{y_i}\right)} +  \frac{\xi}{\sqrt{TK}} \sum_{i=1}^{TK}\sqrt{y_i{\log\left(1 + \frac{1}{y_i}\right)}}\right)\\
%     &\geq \frac{1}{\sqrt{K}} \left(\sum_{i=1}^{TK}{\log \left(1+\frac{1}{y_i}\right)} + {\xi}{y_i{\log\left(1 + \frac{1}{y_i}\right)}}\right)\\
%     &\geq \frac{1}{\sqrt{K}} \left(\sum_{i=1}^{TK} \log\left(1 + \frac{1}{y_i}\right)\big(1 + \xi y_i\big) \right)\\
%     &\geq \frac{1}{\sqrt{K}} \left(\sum_{i=1}^{TK} \frac{\frac{1}{y_i}}{1 + \frac{1}{y_i}}\big(1 + \xi y_i\big) \right)\\
%     &= \frac{1}{\sqrt{K}}\left(\sum_{i=1}^{TK}\frac{1 + \xi y_i}{1 + y_i} \right)\\
%     &\geq T \sqrt{K} {\xi}.
% \end{align*}
% Recall that $\xi = \underset{i}{\min} (u_i^T\bh)^2$. Now, consider an $\bh$ that makes a $\pi/4$ angle with all the eigen-vectors $u_i$, $i\in[TK]$ and therefore $\xi = \frac{1}{\sqrt{2}}$. Note that for the positive definite assumption of NTK to hold, all the contexts need to be distinct and therefore we can always choose such an $h$. In such a case, the regret bound for NeuralUCB is $\bnucb(T,\lambda) = \Omega(T)$ which is meaningless.
% \end{proof}
% \begin{remark}
%     Note that the $\Omega(T)$ regret holds for any $\bh$ whose dot product with all the eigen vectors of $\bH$ is lower bounded by a constant.
% \end{remark}
% \begin{proposition}
% \label{prop:nucb_2}
%     For any cumulative reward vector $\bh$, with $\kappa$ as the condition number of the NTK matrix, the regret bound for NeuralUCB is 
%     \[\emph{$\bnucb$}(\lambda,T) \geq \displaystyle\frac{\|\bh\|_2}{\sqrt{\kappa}}\sqrt{K}T.\]
% \end{proposition}
% \begin{proof}
% Using the same notation as in the previous section, we can lower bound $S$ and $\Tilde{d}$ as follows:
% \begin{align*}
%     S &\geq \sqrt{\lambda_{\min}(\bH^{-1})\|\bh\|_{2}^2} = \frac{1}{\sqrt{\lambda_{\max}(\bH)}}\|\bh\|_{2}\\
%     \tilde{d} = \frac{\log \det(\bI+\bH/\lambda)}{\log(1+TK/\lambda)} &\geq \frac{\log\left(\lambda_{\min}\left(\bI + \bH/\lambda\right)^{TK}\right)}{\log\left(1+TK/\lambda\right)} \geq TK \frac{\log(1 + \frac{\lambda_0}{\lambda})}{\log\left(1+\frac{TK}{\lambda}\right)}
% \end{align*}
% Using these we can lower bound $\bnucb(T,\lambda)$ as follows:
% \begin{align*}
%     \bnucb(T,\lambda) &\geq \sqrt{T} \Bigg( TK \frac{\log(1 + \frac{\lambda_0}{\lambda})}{\log\left(1+\frac{TK}{\lambda}\right)}\log\left(1+\frac{TK}{\lambda}\right) \\
%     &\qquad\qquad + \|\bh\|_{2}\sqrt{TK \frac{\lambda}{\lambda_{\max}(H)}\frac{\log(1 + \frac{\lambda_0}{\lambda})}{\log\left(1+\frac{TK}{\lambda}\right)}\log\left(1+\frac{TK}{\lambda}\right)} \Bigg)\\
%     &= T\sqrt{K} \left( \sqrt{TK}\log\left(1 + \frac{\lambda_0}{\lambda}\right) + \frac{\|\bh\|_{2}}{\sqrt{\kappa}}\sqrt{\frac{\lambda}{\lambda_0}\log\left(1 + \frac{\lambda_0}{\lambda}\right)} \right)\\
%     &= T\sqrt{K} \left(\sqrt{TK}\log\left(1 + \frac{1}{y}\right) + \frac{\|\bh\|_{2}}{\sqrt{\kappa}}\sqrt{y\log\left(1 + \frac{1}{y}\right)} \right),
% \end{align*}
% where $y = \frac{\lambda}{\lambda_0}$ and $\kappa = \frac{\lambda_{\max(H)}}{\lambda_{\min}(H)}$ is the condition number of of the NTK. Since $y\log(1 + \frac{1}{y}) \leq 1$ and for $T,K \geq 1$, we have
% \begin{align}
%     \bnucb(T,\lambda) &\geq T\sqrt{K} \left( \log\left(1 + \frac{1}{y}\right) \left(1 + \frac{y\|\bh\|_{2}}{\sqrt{\kappa}}\right) \right) \\
%     &\geq T\sqrt{K} \left(\frac{1+\frac{\|\bh\|_{2}}{\sqrt{\kappa}}y}{1+y} \right)\\
%     &\geq T \sqrt{K} \frac{\|\bh\|_{2}}{\sqrt{\kappa}}
% \end{align}
% If $\kappa$ and $\|\bh\|$ are $\Theta(1)$, $\bnucb(T,\lambda)$ is $\Omega(T)$.
% \end{proof}

% \subsection{\texorpdfstring{$\Omega(T)$}{alpha} regret for Neural Thompson Sampling \citep{zhang2021neural}}
% The bound on the regret for Neural Thompson sampling is given by (ignoring constants):
% \begin{align*}
%     \reg(T) &\leq \sqrt{T}(1 + \sqrt{\log T + \log K}) \left(S + \sqrt{\tilde{d} \log(1+TK/\lambda)}\right)\sqrt{\lambda\tilde{d}\log(1 + TK)}\\
%     % &= \sqrt{T} (1 + \sqrt{\log T + \log K}) \left(S\sqrt{\lambda\tilde{d}\log(1 + TK)} + \tilde{d}\sqrt{\lambda \log(1+TK/\lambda)\log(1 + TK)} \right)\\
%     &:= B(T)
% \end{align*}
% We present two lower bounds on $\bnts(T)$ below. As in NeuralUCB, the first result is an existential result and the second result provides an $\Omega(T)$ bound for any reward function and set of context vectors as long as $\|\bh\|_2$ and $\lambda_0$ are $\Theta(1)$. 

% \begin{proposition}
% \label{prop:nts_1}
%     There exists a reward vector $\bh$ such that the regret bound for NeuralUCB is lower bounded as
%     \[\emph{$\bnucb$}(\lambda,T) \geq \displaystyle\frac{1}{2\sqrt{2}}\sqrt{K}T.\]
% \end{proposition}
% \begin{proof}
% For Neural Thompson sampling the regularization parameter $\lambda$ is chosen to be $\lambda = 1 + 1/T$ (see Theorem 3.5 in \citet{zhang2021neural}) and therefore $1 \leq \lambda \leq 2$ for any $T\geq 1$. 
% Therefore we can lower bound the effective dimension as,
%     \begin{align*}
%     \tilde{d} &= \frac{\log \det(\bI+\bH/\lambda)}{\log(1+TK/\lambda)} = \frac{\log \left(\displaystyle\prod_{i=1}^{TK}\left(1+\frac{\lambda_{i}(\bH)}{\lambda}\right)\right)}{\log(1+TK/\lambda)} = \frac{\displaystyle \sum_{i=1}^{TK}\log  \left(1+\frac{\lambda_{i}(\bH)}{\lambda}\right)}{\log (1+{TK}/{\lambda})}
%     \geq \frac{\displaystyle \sum_{i=1}^{TK} \log  \left(1+\frac{\lambda_{i}(\bH)}{2}\right)}{\log (1+{TK})}
% \end{align*}
% \begin{align*}
%     \bnts(T) &\geq \sqrt{T}\left(
%     \sqrt{\bh^T \bH^{-1}\bh}\sqrt{\displaystyle \sum_{i=1}^{TK} \log \left(1+\frac{\lambda_{i}(\bH)}{2}\right)} + \sum_{i=1}^{TK} \log\left(1+\frac{\lambda_{i}(\bH)}{2}\right)
%     \right)\\
%     &\geq \sqrt{T} \left(\xi \sqrt{\sum_{i=1}^{TK}\frac{1}{\lambda_{i}(\bH)}\sum_{i=1}^{TK} \log\left(1+\frac{\lambda_{i}(\bH)}{2}\right)} + \sum_{i=1}^{TK} \log\left(1+\frac{\lambda_{i}(\bH)}{2}\right)
%     \right)\\
%     &\geq \sqrt{T} \left( \xi \sqrt{\sum_{i=1}^{TK} y_i \log\left(1 + \frac{1}{2y_i}\right)} + \sum_{i=1}^{TK} \log\left(1+\frac{1}{2y_i}\right)\right)\\
%     &\geq \sqrt{T} \left( \xi \frac{1}{\sqrt{TK}} \sum_{i=1}^{TK} \sqrt{y_i \log\left(1+\frac{1}{2y_i}\right) } + \sum_{i=1}^{TK} \log\left(1+\frac{1}{2y_i}\right) \right)\\
%     &\geq \sqrt{T} \left( \frac{1}{\sqrt{TK}} \sum_{i=1}^{TK} \xi y_i \log \left( 1 + \frac{1}{2y_i}\right) + \log \left( 1 + \frac{1}{2y_i}\right)  \right)\\
%     &= \sqrt{T} \left( \frac{1}{\sqrt{TK}} \sum_{i=1}^{TK} \log \left( 1 + \frac{1}{2y_i}\right) (1+\xi y_i) \right)\\
%     &\geq \sqrt{T} \left( \frac{1}{\sqrt{TK}} \sum_{i=1}^{TK} \frac{1/2y_i}{1 + 1/2y_i}(1+\xi y_i) \right)\\
%     &= \sqrt{T} \left( \frac{1}{\sqrt{TK}} \sum_{i=1}^{TK} \frac{1+\xi y_i}{1 + 2y_i} \right)\\
%     &\geq \sqrt{T} \frac{1}{\sqrt{TK}} TK \frac{\xi}{2}\\
%     &= T\sqrt{K}\frac{\xi}{2}. 
% \end{align*}
% As in the proof of Proposition~\ref{prop:nucb_1}, for $\bh$ making an angle of $\pi/4$ with all eigen-vectors of $\bH$, $\xi \geq \frac{1}{\sqrt{2}}$, which proves the claim.

% \begin{proposition}
%     For any cumulative reward vector $\bh$, the regret bound for Neural Thompson sampling is 
%     \[\emph{$\bnts$}(\lambda,T) \geq T\sqrt{T}K \frac{\lambda_0}{2 + \lambda_0}\]
% \end{proposition}
% Recall, $1 \leq \lambda \leq 2$ for any $T\geq 1$, and therefore we can lower bound the effective dimension as,
% \begin{align*}
%    \tilde{d} = \frac{\log \det (I + \bH/\lambda)}{\log (1 + TK/\lambda)} \geq  \displaystyle  TK \frac{\log (1 + {\lambda_0}/{\lambda})}{\log(1 +  TK/\lambda)} \geq TK \frac{\log (1 + {\lambda_0}/{\lambda})}{\log(1 +  TK)}
% \end{align*}
% Therefore, using $1 \leq \lambda \leq 2$ and $S\geq \sqrt{\bh^T \bH^{-1}\bh}$,
% \begin{align*}
%     \bnts(T) &\geq \sqrt{T}\left(\sqrt{\bh^T \bH^{-1}\bh} + \sqrt{TK \log(1 + \lambda_0/2)}\right)\sqrt{TK \log(1+\lambda_0/2) }\\
%     &\geq T\sqrt{T}K\log(1+\lambda_0/2)\\
%     &\geq T\sqrt{T}K\frac{\lambda_0/2}{1 + \lambda_0/2}\\
%     &\geq T\sqrt{T}K \frac{\lambda_0}{2 + \lambda_0}
% \end{align*}
% If $\lambda_0 = \Theta(1)$, $\bnts(T)$ is $\Omega(T)$.
% % \begin{align*}
% %     B(T) &\geq {T}\sqrt{K}\sqrt{\bh^T \bH^{-1}\bh}\sqrt{\displaystyle \sum_{i=1}^{TK} \log \left(1+\frac{\lambda_{i}(H)}{2}\right)}\\
% %     &\geq T\sqrt{K}\xi \sqrt{\sum_{i=1}^{TK}\frac{1}{\lambda_{i}(\bH)}\displaystyle \sum_{i=1}^{TK} \log \left(1+\frac{\lambda_{i}(H)}{2}\right)}\\
% %     &\geq T\sqrt{K}\xi \sqrt{\sum_{i=1}^{TK} y_i\log \left(1 + \frac{1}{2y_i} \right)}\\
% %     &= T\sqrt{T} \xi \frac{1}{\sqrt{TK}}\\
% %     &\geq T\sqrt{T} \xi \frac{1}{\sqrt{KT}} \sum_{i=1}^{KT}\sqrt{y_i \log \left(1 + \frac{1}{2y_i} \right)}\\
% %     &\geq T\sqrt{K}\xi \sqrt{\sum_{i=1}^{TK} y_i \frac{1/2y_i}{1 + 1/2y_i}}
% % \end{align*}

% \end{proof}

==> app/app_prelims.tex <==

% Before we proceed with the proof of the claims in Section~\ref{sec:Neural_online_learning_formulation} and Section~\ref{sec:Neural_online_learning_regret}, we state a few recent results from \citet{banerjee2023restricted} that we will use throughout our proofs. Before proceeding, we put the initialization of the feedforward network discussed after \eqref{eq:specball} formally as an assumption. 
% \begin{asmp}
% For the feedforward model in \eqref{eq:DNN_smooth}, the weights are initialized as $w_{0,ij}^{(l)} \sim \cN(0,\sigma_0^2)$ for $l\in[L]$ where $\sigma_0 = \frac{\sigma_1}{2\left(1 + \frac{\sqrt{\log m}}{\sqrt{2m}}\right)}, \sigma_1 > 0$, and $\v_0$ is a random unit vector with $\norm{\v_0}_2=1$.
% \label{asmp:actinit}
% \end{asmp}
% We also define \abcomment{why equation without a number+label, we must be using it somewhere}
% \begin{align*}
%     K_{\ntk}(i,j;\theta_t) = \Big\langle\nabla_{\theta}{f}(\theta;\x_{t,i}), \nabla_{\theta}{f}(\theta;\x_{t,j}) \Big\rangle
% \end{align*}
% and the NTK matrix $K_{\ntk}(\theta_t) = [K_{\ntk}(i,j;\theta_t)]$.
% \begin{restatable}[\textbf{Hessian Spectral Norm Bound}]{lemm}{boundhess}
% \label{theo:bound-Hess}
% Under Assumptions~\ref{asmp:smooth} and \ref{asmp:actinit}, for any $\x \in \cX$, $\theta \in B_{\rho,\rho_1}^{\spec}(\theta_0)$, {$\rho_1=O(\poly(L))$},  with probability at least $(1-\frac{2(L+1)}{m})$, we have 
% \begin{equation}
% \label{eq:bound_Hessian}
%    \norm{ \nabla^2_\theta f(\theta;\x)}_2 \leq \frac{c_H}{\sqrt{m}}\quad \text{and} \quad \| \nabla_{\theta} f(\theta;\x) \|_2 \leq \varrho~,
% \end{equation}
% with $c_H = \cO(\poly(L)(1+\gamma^{2L}))$ where $\gamma := \sigma_1 + \frac{\rho}{\sqrt{m}}$ and $\varrho = \cO(1)$. \abcomment{not precise enogh, show the form in terms of $\rho, \rho_1$ as equation, will be useful elsewhere.} 
% \end{restatable}

% \begin{restatable}[\textbf{Loss bounds}]{lemm}{lemLbounds}
% Under Assumptions~\ref{asmp:smooth} and \ref{asmp:actinit}, for $\gamma = \sigma_1 + \frac{\rho}{\sqrt{m}}$, each of the following inequalities hold with probability at least $\left(1-\frac{2(L+1)}{m}\right)$: 
% $\cL(\theta_0)\leq c_{0,\sigma_1}$ and 
% $\cL(\theta)\leq c_{\rho_1,\gamma}$ 
% for $\theta \in B_{\rho,\rho_1}^{\spec}(\theta_0)$, where $c_{a,b}=\frac{2}{N}\sum^N_{i=1}y_i^2+2(1+a)^2|g(b)|^2$ and $g(a)=a^L+|\phi(0)|\sum^L_{i=1}a^i$ for any $a,b\in\R$.
% \label{lem:BoundTotalLoss}
% %\vspace*{-2mm}
% \end{restatable}
% %

% \begin{restatable}[\textbf{Loss gradient bound}]{lemm}{corrtotalbnd}
% \label{cor:total-bound}
% Under Assumptions~ \ref{asmp:smooth} and \ref{asmp:actinit}, for $\theta \in B_{\rho,\rho_1}^{\spec}(\theta_0)$, with probability at least $\left(1-\frac{2(L+1)}{m}\right)$, we have
% $\|\nabla_\theta \cL(\theta)\|_2  \leq 2\sqrt{\cL(\theta)}\varrho\leq 2\sqrt{c_{\rho_1,\gamma}}\varrho$,
% %\end{align}
% with $\varrho$ as in Lemma~\ref{theo:bound-Hess} and $c_{\rho_1,\gamma}$ as in Lemma~\ref{lem:BoundTotalLoss}.
% \end{restatable}



% \begin{restatable}[\textbf{Local Smoothness}]{lemm}{theosmoothnes}
% Under Assumptions~ \ref{asmp:smooth} and \ref{asmp:actinit}, with probability at least $(1 - \frac{2(L+1)}{m})$, $\forall \theta,\theta' \in B_{\rho,\rho_1}^{\spec}(\theta_0)$, 
% %
% \begin{equation}
% \label{eq:Smooth-formula-NN}
% \begin{split}
% \hspace*{-5mm} 
% \cL(\theta') & \leq \cL(\theta) + \langle \theta'-\theta, \nabla_\theta\cL(\theta) \rangle + \frac{\beta}{2} \| \theta' - \theta \|_2^2~, \quad
% \text{with} \quad
% \beta = b\varrho^2 + \frac{c_H\sqrt{c_{\rho_1,\gamma}}}{\sqrt{m}} ~,
% \end{split}
% \end{equation}
% %
% with $c_H$ as in~Lemma~\ref{theo:bound-Hess}, $\varrho$ as in Lemma~\ref{theo:bound-Hess}, and $c_{\rho_1,\gamma}$ as in Lemma~\ref{lem:BoundTotalLoss}. Consequently, $\cL$ is locally $\beta$-smooth. 
% \label{theo:smoothnes}
% \end{restatable}




==> sec/Bandit_regret.tex <==
% In this section we use our regret bounds from Section~\ref{sec:Neural_online_learning_regret} to provide regret bounds in the contextual bandit setting for $\mathtt{NeuRIG}$ and $\mathtt{NeuR^2IG}$. The proof of all the claims have been pushed to Appendix.

% \abcomment{Are the regret bounds really possible without the interpolation result introduced in Theorem 2.1.} 

% \abcomment{Is there any relation between $L^*$ and $\inf_{\theta} \sum_t \cL(\theta;\z_t)$}

% % \subsection{Regret bounds for $\mathtt{NeuRIG}$}

% \subsection{Regret bounds for \texorpdfstring{$\mathtt{NeuRIG}$}{}}

% In the linear setting i.e., when $h(\x_{t,a})$ is a linear function of $\x_{t,a}$, choosing Vovk-Azoury-Warmuth forecaster \cite{Azoury} leads to 
% $R_{Sq}(T) \leq p \log(T/p)$ where $p$ is the dimension of the features (or number of parameters) and thus in the bandit setting gives a regret bound of $R(T) = O(\sqrt{pKT} \log(T/p))$. However, when the function class is parameterized with a neural network a regret bound with number of parameters ($p=mL$ in our notation) is essentially useless. 
% Using online gradient descent with a neural network and using a naive analysis that exploits almost convexity of the loss function would lead to a regret of $R_{Sq}(T) = \mathcal{O}(\sqrt{T})$ for online regression and a regret of $\reg(T) = \tilde{\mathcal{O}}(T^{3/4})$ in the bandit setting. Note that such an analysis does not exploit the sharp regret bounds we obtained in Section~\ref{subsec:sq_loss}. The following result formalizes this regret bound:
% \begin{restatable}[\textbf{Basic Regret bound for $\mathtt{NeuRIG}$}]{theo}{Neurigbasicregret}
% \label{thm:Neurig_basic_regret}
%     Under Assumption~\ref{asmp:realizability_bandit} and \ref{asmp:NTK_bandit} the regret for $\mathtt{NeuRIG}$ without regularization is bounded as: w.p. $1-\delta$,\rdcomment{Choice of $m$}
%     \begin{align*}
%         \reg(T) \leq \cO(\sqrt{K}T^{3/4})
%     \end{align*}
% \end{restatable}
% Our objective is to obtain a regret of the form $\tilde{\mathcal{O}}(\sqrt{T})$, that does not depend on the number of parameters in the neural network. The following Theorem provides such a regret bound using the regret bounds obtained for online regression in Section~\ref{sec:Neural_online_learning_regret}.
% \begin{restatable}[\textbf{Main Regret bound for $\mathtt{NeuRIG}$}]{theo}{Neurigmainregret}
% \label{thm:Neurig_main_regret}
%     Under Assumption~\ref{asmp:realizability_bandit} and \ref{asmp:NTK_bandit} the regret for $\mathtt{NeuRIG}$ is bounded as: w.p. $1-\delta$,\rdcomment{Choice of $m$}
%     \begin{align*}
%         \reg(T) \leq \tilde{\cO}(\sqrt{KT})
%     \end{align*}
% \end{restatable}


% \subsection{Regret bounds for \texorpdfstring{$\mathtt{NeuR^2IG}$}{}}

% As in the previous subsection we first present a sub-optimial regret bound  for $\mathtt{NeuR^2IG}$ that does not use the regret bound with KL-loss developed in Section~\ref{subsec:kl_loss}. Here, $L^*$ is the loss of the best policy and is formally defined as $L^* = \sum_{t=1}^{T} y_{t,a_t^*}$
% \begin{restatable}[\textbf{Basic Regret bound for $\mathtt{NeuR^2IG}$}]{theo}{Neur2igbasicregret}
% \label{thm:Neur2ig_basic_regret}
%     Under Assumption~\ref{asmp:realizability_bandit} and \ref{asmp:NTK_bandit} the expected regret for $\mathtt{NeuRIG}$ without regularization is bounded as\rdcomment{Choice of $m$}
%     \begin{align*}
%         \Ex[\reg(T)] \leq \cO(\sqrt{L^*KT})
%     \end{align*}
% \end{restatable}
% Next, we present a regret bound of the form $\tilde{\mathcal{O}}(\sqrt{L^*})$, that does not depend on the number of parameters in the neural network and depends on the time horizon $T$ at most logarithmically. 
% \begin{restatable}[\textbf{Main Regret bound for $\mathtt{NeuRIG}$}]{theo}{Neurigmainregret}
% \label{thm:Neurig_main_regret}
%     Under Assumption~\ref{asmp:realizability_bandit} and \ref{asmp:NTK_bandit} the regret for $\mathtt{NeuRIG}$ is bounded as,\rdcomment{Choice of $m$}
%     \begin{align*}
%         \Ex[\reg(T)] \leq \tilde{\cO}(\sqrt{L^*K})
%     \end{align*}
% \end{restatable}

% % Therefore we focus on online regression with neural networks in Section \ref{sec:Neural_online_learning}.


% % In this section, we turn to see how our regret bounds from online learning in Section \ref{sec:Neural_online_learning} can be instantiated to obtain instance-dependent bounds for the contextual bandit problem. 

% % Our first step will be to use a reduction from contextual bandit to online learning, following the work of~\cite{foster2020beyond, foster2021efficient}. %We adapt the reweighted inverse gap weighting algorithm with a neural model, which we term neural reweighted inverse gap weighting\szcomment{insert acronym here}. The algorithm is summarized in~\cref{algo:neural-rigw}. 
% % We show how the reweighted inverse gap weighting algorithm from~\cite{foster2021efficient} can be adapted to work with overparameterized neural networks and give sharp regret bounds while leveraging the representation power of neural networks.
% % \subsection{Regret Bounds with Squared error loss}
% % \begin{theo}
% % Regret bounds for neural bandits with Smooth

% % \[
% % \begin{aligned}
% % R(T)\leq &  O(\sqrt{K}T^{3/4}) +       O(\sqrt{K T ( 2 \sum_{t=1}^T  \cL(\theta^*;\z_t)})  + \mathcal{O}( \sqrt{KT \log (2 \delta^{-1})} ) 
% % \end{aligned}
% % \]

% % \end{theo}






% \iffalse
% Following the result in~\cite{foster2021efficient}, we have the following regret bound for the contextual bandit problem. Recall $H_T = (\z_1, ..., \z_T)$ is the history of the learner. Let $L^* = \sum_{t=1}^Ty_{t,a_t^*}$ represent the optimal loss. 
% \begin{proposition}
% \[
% \Ex[\RegCB(T)] \le O(\sqrt{KL^* \cdot \RegKL(H_T)} + K\RegKL(H_T)). 
% \]
% \end{proposition}

% \begin{remark}
% Our regret bound takes the same form as~\cite{foster2021efficient}. However, the regret bound replaces $\RegKL$ in~\cite{foster2021efficient} by the instance-dependent regret term $\RegKL(H_T)$. 
% \end{remark}

% \fi


% %We now show how our regret bounds for the online learning problem in previous section translates to a $O(K\log T)$ regret in the bandit multi-class classification problem. 

% \iffalse


% The bandit classification problem is defined as follows. At each round $t\in [T]$, a training data $x_t\in \bbR^d$ is presented to the learner to be classified in one of $K$ classes. The learner predicts a class and suffers loss 1 if the prediction is incorrect, and suffers loss 0 if the prediction is correct. In other words, the learner will only be able to learn whether his prediction was correct or not, and will not learn the true label if his prediction is incorrect. 

% We can recast the bandit multi-class classification problem into our adversarial contextual bandit setting. At round $t$, when the training data is $x\in \bbR^{d}$, it is transformed into $K$ arms, $x_{t,1} = (x^\top, \bm{0}, \dots, \bm{0})^\top, x_{t,2} = (\bm{0}, x^\top, \dots, \bm{0})^\top, \dots, x_{t,K} = (\bm{0}, \bm{0}, \dots, x^\top)^\top$, 
% matching $K$ classes in sequence. When the true label of $x$ is class $k$, the losses are given by
% \begin{align*}
% y_{t, k} &= 0\\
% y_{t, k'} &= 1\quad \forall k'\neq k. 
% \end{align*} 

% \fi









% \iffalse
% \begin{theo}
% \label{thm:banditKL}
% Using~\cref{algo:neural-rigw} with $\gamma = \Theta(K)$,
% \[
% \Ex[\RegCB(T)] = O(K\sum_{t=1}^T \cL_t(\theta_t; \z_t) + K\log T)
% \]
% \end{theo}
% \begin{proof}
% Note in the bandit classification problem $L^* = 0$,
% since the optimal loss suffered through $T$ rounds is $0$, as each context will belong to some class that gives loss 0 at each round. 

% Hence the desired result comes from the following: 
% \begin{align*}
% \Ex[\RegCB] &\le O(K\RegKL(H_T)) \\
% &\le O(\inf_{\theta\in \Ball(\theta_1, R)} K\sum_{t=1}^T \cL(\theta; z_t) + K \log T)
% \end{align*}
% The first line follows from~\cref{thm:banditKL} and the second line follows from~\cref{thm:PLregret}. 
% \end{proof}
% \fi



% % \begin{restatable}{theo}{banditregretsmooth}
% % Regret bounds for neural bandits with Smooth

% % \[
% % \begin{aligned}
% % R(T)\leq & O(\sqrt{K T ( 2 \sum_{t=1}^T  \cL(\theta^*;\z_t) + O(\log T)    )})
% % & + O( \sqrt{KT \log (2 \delta^{-1})} ) 
% % \end{aligned}
% % \]



% % \end{restatable}


% % \begin{remark}
% % Our regret bound does not make any distributional assumption on the data nor the label: the input data and label can be adversarially chosen, and our algorithm adapts organically to the data-dependent complexity term $\sum_{t=1}^T \cL_t(\theta^*; \z_t)$. This term can be understood as a measure as to how easily the data can be classified. When the data can be easily classfied, as measured by the RKHS norm $\sqrt{y \Theta^{-1} y}$ in the NTK induced kernel space~\cite{cao2019generalization, arora2019fine}, our algorithm only makes $O(K\log T)$ number of mistakes.
% % \end{remark}



% % \begin{remark}
% % Discuss the difference of these regret bounds from existing works.
% % \end{remark}

% % \subsection{Regret Bounds with KL loss}

% % \begin{theo}
% % Regret bounds for neural bandits with Smooth activaltion and KL loss


% % \begin{align*}
% %     \E [R(T)] \leq \mathcal{O}(\sqrt{L^* K }T^{1/4}) + \mathcal{O}(K \sqrt{T}),
% % \end{align*}

% % \end{theo}

==> sec/High_prob_regret.tex <==

In this section we show that with some extra computation we can also obtain high probability regret bounds.
Let ${\epsvec}_s = (\varepsilon_{s,1},\varepsilon_{s,2},\ldots,\varepsilon_{s,p})^T$ where each $\varepsilon_{s,i}$ is drawn iid from a Rademacher distribution. Consider $S$ such iid draws $\{{\epsvec}_s\}_{s=1}^S$, and 
define the following function
\begin{align}
    \label{eq:ftildeS}
    \tilde{f}^{(S)}\left(\theta;\x_{t,i},{\epsvec}^{(1:S)}\right) = \frac{1}{S} \sum_{s=1}^S\tilde{f}(\theta;\x_{t,i},{\epsvec}_{s}),
\end{align}
where $\tilde{f}(\theta;\x_{t,i},{\epsvec}_{s})$ is as defined in \eqref{eq:output_reg_def}. The square loss function  with the above predictor is given by
\begin{align}
    \label{eq:combined_loss}
    \cL_{\sq}\left(y_t,\tilde{f}^{(S)}\big(\theta;\x_{t},{\epsvec}^{(1:S)}\big)\right) =  \frac{1}{n_t}\sum_{i=1}^{n_t} \ell_{\sq}\left(y_{t,i},\tilde{f}^{(S)}\big(\theta;\x_{t,i},{\epsvec}^{(1:S)}\big)\right)
\end{align}
The proof of all the auxiliary lemmas are in Appendix~\ref{sec:app_online_reg_whp}.
\begin{restatable}[\textbf{High Probability Regret Bound for Squared Loss}]{theo}{hpthmregsq}
    \label{thm:hp_reg_sq_loss_online}
     Under assumption \ref{asmp:ntk} with appropriate choice of step-size sequence $\{\eta_t\}$, width $m$ and regularization constant $c_{\rg}$, with high probability over the randomness of initialization and $\{\varepsilon_i\}_{i=1}^{p}$, the regret of Algorithm~\ref{algo:onlineneural} with loss $\cL_{\sq}\left(y_t,\tilde{f}^{(S)}\big(\theta;\x_{t,i},{\epsvec}^{(1:S)}\big)\right)$, $S = \Theta(\log m)$ and projection ball $\ballfrob$ with $\rho = \Theta(\sqrt{N}/\lambda_0)$ and $\rho_1 = \Theta(1)$ is given by
    \begin{align*}
        \emph{$\Rsq(T)$} \leq \cO(\log T),
    \end{align*}
\end{restatable}
\emph{Proof.}
Before proceeding with the proof we define the following average loss function
\begin{align}
\label{eq:avg_loss}
    \cL_{\sq}^{(S)}\Big(y_t,\big\{\tilde{f}(\theta;\x_t,\epsvec_s)\big\}_{s=1}^{S}\Big) = \frac{1}{S}\sum_{s=1}^S \cL_{\sq}\left(y_t,\tilde{f}(\theta;\x_t,\epsvec_s)\right).
\end{align}
Note that since $\ell_{\sq}$ is convex in the second argument using Jensen we have
\begin{align*}
    \ell_{\sq}\left(y_{t,i},\tilde{f}^{(S)}\big(\theta;\x_{t,i},{\epsvec}^{(1:S)}\big)\right) = \ell_{\sq}\left(y_{t,i},\frac{1}{S} \sum_{s=1}^S\tilde{f}(\theta;\x_{t,i},{\epsvec}_{s})\right) \leq \frac{1}{S} \sum_{s=1}^S \ell_{\sq}\left(y_{t,i},\tilde{f}(\theta;\x_{t,i},{\epsvec}_{s})\right)
\end{align*}
Combining this with $\eqref{eq:combined_loss}$ we get
\begin{align*}
    \cL_{\sq}\left(y_t,\tilde{f}^{(S)}\big(\theta;\x_{t},{\epsvec}^{(1:S)}\big)\right) &\leq \frac{1}{n_t}\sum_{i=1}^{n_t} \frac{1}{S}\sum_{s=1}^S \ell_{\sq}\Big(y_{t,i},\tilde{f}\big(\theta;\x_{t,i},{\epsvec}_{s}\big)\Big) \\
    &= \frac{1}{S}\sum_{s=1}^S \cL_{\sq}\left(y_t,\tilde{f}(\theta;\x_t,\epsvec_s)\right) = \cL_{\sq}^{(S)}\Big(y_t,\big\{\tilde{f}(\theta;\x_t,\epsvec_s)\big\}_{s=1}^{S}\Big)
\end{align*}
Therefore bounding the regret with the average loss $\eqref{eq:avg_loss}$ would imply a regret with the loss defined in $\eqref{eq:combined_loss}$. 
As in proof of Theorem~\ref{thm:reg_sq_loss_online} the proof the current theorem follows along the following four steps.
\begin{enumerate}
    \item[\textbf{1.}] \textbf{Square loss} $\ell_{sq}$ \textbf{is lipschitz, strongly convex and smooth wrt the output with high probability.}
    
    We show that the loss function $\ell_{\sq}$ is lipschitz, strongly convex and smooth with respect to the output $\tilde{f}(\theta;\x)$ inside $\ballfrob$ with high probability over the randomness of initialization and $\{\varepsilon_i\}_{i=1}^{p}$.
    \begin{restatable}[]{lemmma}{hpsqlemmaone}
    \label{lemma:hp_sq_loss_lip_sc}
    For $\theta \in \ballfrob$, with probability $\left(1-\frac{2N(L+1)+1}{m}\right)$ over the randomness of initialization and $\{\varepsilon_i\}_{i=1}^{p}$, the loss function $\ell_{\sq}\Big(y_{t,i},\tilde{f}^{(S)}\left(\theta;\x_{t,i},{\epsvec}^{(1:S)}\right)\Big)$ is lipschitz, strongly convex and smooth with respect to the output $\tilde{f}^{(S)}\left(\theta;\x_{t,i},{\epsvec}^{(1:S)}\right)$. Further the parameters $\lambda_{\sq},a_{\sq}$ and $b_{\sq}$ are $\Theta(1)$.
    \end{restatable} 
    
    \item[\textbf{2.}] \textbf{The average loss at stage} $t \in [T]$, $\cL_{\sq}^{(S)}\Big(y_t,\big\{\tilde{f}(\theta;\x_t,\epsvec_s)\big\}_{s=1}^{S}\Big)$ \textbf{has a unique minimizer.}
    
    We show that $\cL_{\sq}^{(S)}\Big(y_t,\big\{\tilde{f}(\theta;\x_t,\epsvec_s)\big\}_{s=1}^{S}\Big)$ is strongly convex with respect to the parameters $\theta \in\ballfrob$ at every $t\in [T]$ and therefore has a unique minima. 
    \begin{restatable}[]{lemmma}{hpsqlemmatwo}
        \label{lemma:sq_sc}
        Under Assumption \ref{asmp:ntk} and $c_{\rg} = \sqrt{8\lambda_{\sq}C_H}$, with probability $\left(1-\frac{2N(L+2)}{m}\right)$ over the randomness of the initialization and $\{\epsvec_s\}_{s=1}^S$, $\cL_{\sq}^{(S)}\Big(y_t,\big\{\tilde{f}(\theta;\x_t,\epsvec_s)\big\}_{s=1}^{S}\Big)$ is $\nu$-strongly convex with respect to $\theta \in \ballfrob$, where $\nu = \mathcal{O}\left(\frac{1}{\sqrt{m}}\right).$
    \end{restatable}
    
    \item[\textbf{3.}] \textbf{The average loss at stage} $t \in [T]$, $\cL_{\sq}^{(S)}\Big(y_t,\big\{\tilde{f}(\theta;\x_t,\epsvec_s)\big\}_{s=1}^{S}\Big)$ \textbf{satisfies the QG condition.}
    
    We show that the loss $\cL_{\sq}^{(S)}\Big(y_t,\big\{\tilde{f}(\theta;\x_t,\epsvec_s)\big\}_{s=1}^{S}\Big)$ satisfies the QG condition in Assumption~\ref{asmp:qg} with high probability over the randomness of initialization and almost surely (a.s.) over the randomness of $\epsvec$.
    \begin{restatable}[]{lemmma}{hpsqlemmathree}
        \label{lemma:QG_sq_loss_lemma}
        Under Assumption~\ref{asmp:ntk} with probability $\left(1-\frac{4N(L+1)}{m}\right)$ over the randomness of the initialization $\cL_{\sq}^{(S)}\Big(y_t,\big\{\tilde{f}(\theta;\x_t,\epsvec_s)\big\}_{s=1}^{S}\Big)$ satisfies the QG condition almost surely over the randomness of $\{\varepsilon_i\}_{i=1}^{p}$, with constant $\mu = \lambda_0/2n_t$.
    \end{restatable}
    
    \item[\textbf{4.}] \textbf{Bounding the final regret.}
    
    
    % The above three steps ensure that all the assumptions of Theorem~\ref{thm:PLregret} are satisfied for the expected loss $\E_{\epsvec}\losstildesq{\theta}$. Therefore invoking Theorem~\ref{thm:PLregret} we get and using the fact that $m = \Omega(N^5/\lambda_0^6)$
    % \begin{gather}
    % \label{eq:final_regret_exp}
    %     \sum_{t=1}^{T}\E_{\epsvec}\losstildesq{\theta_t} - \E_{\epsvec}\losstildesq{\tilde{\theta}^*} \leq 2 \sum_{t=1}^{T}\E_{\epsvec}\losstildesq{\tilde{\theta}^*} + \cO(\log T).\\
    %     \text{where} \quad \tilde{\theta}^* = \min_{\theta \in \ballfrob} \sum_{t=1}^{T}\E_{\epsvec}\losstildesq{\tilde{\theta}} \nonumber
    % \end{gather}
    % Next we bound $\sum_{t=1}^{T}\E_{\epsvec}\losstildesq{\tilde{\theta}^*}$ using the following lemma.
    % \begin{restatable}[]{lemmma}{sqlemmafour}
    %     \label{lemma:opt_sq_loss_lemma}
    %     Under Assumption~\ref{asmp:real} and \ref{asmp:ntk} with probability $\left(1-\frac{2(L+1)}{m}\right)$ over the randomness of the initialization we have
    %     \begin{align*}
    %         \sum_{t=1}^{T}\E_{\epsvec}\losstildesq{\tilde{\theta}^*} \leq \Theta(1).
    %     \end{align*}
    % \end{restatable}
    % Using Lemma~\ref{lemma:opt_sq_loss_lemma} and $\eqref{eq:final_regret_exp}$ we have $\sum_{t=1}^{T}\E_{\epsvec}\losstildesq{\theta_t} \leq \cO(\log T)$.
    % Finally using the fact that $\min_{\theta \in \ballfrob}\sum_{t=1}^{T}\losssq{\theta} = 0$ from Theorem~\ref{thm:interpolation} we have with high probability over the randomness of initialization $\E_{\epsvec}\big[\Rsq(T)\big]\leq \cO(\log T)$.
    \end{enumerate}
\qed

==> sec/NOR_Formulation0.tex <==
To obtain regret bounds for the contextual bandit setting, we use a reduction from the bandit to the online regression setting in Section \ref{sec:bandit_formulation}. In this and the subsequent section we therefore develop novel regret bounds for the online regression problem with neural models for both squared loss and KL loss and subsequently use these to obtain regret bounds for the bandit problem.


% In Section \ref{sec:bandit_formulation} we saw that to obtain regret bounds for the bandit setting we need to obtain regret bounds for the online regression problem with neural networks. In this section we describe the problem of online regression with neural networks and obtain regret bounds. 

\textbf{Problem Formulation:} At any round $t \in [T] = \{1, \cdots, T\}$, the learner is presented with $n_t$ inputs $\{\x_{t,i}\}_{i=1}^{n_t}$, all drawn from some input space $\cX \subset \bbr^d$ and is required to make real-valued predictions $\hat{y}_{t,i} \in \cY = [0, 1]$ for all $i\in [n_t]$, based on possibly the entire history. Then, the true outcomes $y_{t,i}$ for all $i\in[n_t]$ are observed.  

\begin{asmp} [Realizability]
The conditional distribution of $y_{t,i}$ given $\x_{t,i}$ is defined by some unknown function $h$: $\cX \rightarrow \cY$, such that
\(
\E[y_{t,i} |\x_{t,i}] = h(\x_{t,i}).
\) 
Further w.l.o.g assume the context vectors satisfy $\|\x_{t,i}\| = 1$, $\forall t,i$.
\end{asmp}
We assume that there exists a class of functions $\cF$ from $\cX \rightarrow \cY $, possibly infinite that contains $h$. We are given a loss function $\ell : \cY \times \cY \rightarrow \R$, that measures the error between the prediction $\hat{y}_{t,i}$ and the true output $y_{t,i}$. We will slightly abuse notation and define $\z_t := \{(\x_{t,i}, y_{t,i})\}_{i=1}^{n_t}$ and the cumulative loss as 
\(\cL(\theta_t; \z_t) := \frac{1}{n_t}\sum_{i=1}^{n_t}\ell(y_{t,i}, f(\theta_t;\x_{t,i})),\) where $f \in \cF$ is parameterized by $\theta_t \in \R^p$. 
The regret of online regression is defined as
% With $(x_t)_i = \x_{t,i}$ and $(y_t)_i = y_{t,i}$, the goal of online learning problem is to minimize the \textit{loss regret}:
\begin{equation}
\label{eq:online_reg}
R(T) := \sum_{t =1}^T  \cL(\theta_t; \z_t) - \inf_{f \in \cF} \sum_{t=1}^T \cL(\theta_t; \z_t). 
\end{equation}
% In Section \ref{sec:Neural_online_learning_regret} we provide regret bounds for loss functions satisfying PL type conditions. Subsequently
% we derive regret bounds for specific loss functions, the squared loss and the KL loss.
We will denote $\ell_{t,i} = \ell(y_{t,i},f(\theta_{t}; \x_{t,i})) = \ell(y_{t,i},\hat{y}_{t,i})$, $\ell_{t,i}' = \frac{d \ell_{t,i}}{d \hat{y}_{t,i}}$, and $\ell_{t,i}'' = \frac{d^2 \ell_t}{d \hat{y}^2_{t,i}}$.

% , and denote the history at step $t$ by $H_t := (\x_{1}, y_{1}, ..., \x_{t}, y_{t})$. 



% In contrast with existing works \cite{foster2020beyond, foster2021efficient} that consider finite size of $\cF$ and $h \in \cF$, we do not impose any assumptions on $\cF$ and $h$.
% For the ease of presentation, we restrict $\ell$ to the squared loss function, i.e.,  $\ell(y_t, \hy_t) = (\hy -  y_t )^2$. 


\textbf{Neural Architectures:}
For a suitable non-negative loss function $\ell$, the goal during training (in hindsight) is to minimize the empirical loss: $ \sum_{t=1}^T \cL(\theta_t; \z_t)$, where the prediction $\hat{y}_{t,i} := f(\theta_t;\x_{t,i})$ is from a deep model with parameter $\theta_t\in\R^p$. In our setting, $f$ is a feed-forward multi-layer (fully-connected) neural network with depth $L$, and width $m$ and therefore $p = mL$. We have assumed that the width of all the layers is the same, and that the model has a scalar output, i.e., $f(\theta;\x) \in \R$ for simplicity. We consider two choices of activation functions: 

\rdcomment{should we also provide initialization scheme here?}
\begin{enumerate}
    \item \textbf{Smooth activations:} A neural network with smooth activations with $L$ hidden layers is defined by parameters 
    ${\theta}^\top = ( \vec({W^{(1)}})^\top, ..., \vec({W^{(L)}})^\top, \v^\top)$, where $W^{(l)}, l\in [L]$ represent the weight matrices.  
    Then, the network is computed recursively as: 
    %\hecomment{maybe use the following form instead to be consistent with ReLU?}
    %\bancomment{Yes, good suggestions.}
    \begin{align}
    \label{eq:DNN_smooth}    
    f({\theta}; \x) = \frac{1}{\sqrt{m}} \v^\top\phi\left(\frac{1}{\sqrt{m}}{W}^{(L)}\phi\left(... \phi\left(\frac{1}{\sqrt{m}}{W}^{(1)} \x\right)\ldots\right)\right). 
    \end{align}
    where ${W}^{(1)} \in \bbR^{m \times d}, W^{(l)} \in \R^{m \times m},\forall l \in \{2, \dots, L\}$ are layer-wise weight matrices, $\v\in\R^{m}$ is the last layer vector, $\phi(\cdot )$ is the smooth (pointwise) activation function.
    \item \textbf{ReLU activation. } The neural network with ReLU activation with depth $L$ is defined by parameters 
    ${\theta}^\top = ( \vec({W^{(1)}})^\top, ..., \vec({W^{(L)}})^\top)$, where ${W}^{(1)} \in \bbR^{m \times d}, {W}^{(l)}\in\bbR^{m\times m}, \forall l \in \{2, \dots, L\},    {W}^{(L)}\in\bbR^{1\times m}$, and the neural network function $f$ is defined as
    \begin{align}
    f({\theta}; \x) = \sqrt{m} {W}^{(L)}\phi({W}^{(L-1)}\phi(... \phi({W}^{(1)} \x) ...)). 
    \label{eq:DNN_relu}
    \end{align}
    Here $\phi(x) = \max(x,0)$ denotes the ReLU activation function. 
\end{enumerate}
\textbf{Algorithm} \ref{algo:onlineneural} presents a simple and standard online learning algorithm with gradient descent. Our objective is to bound the regret of this algorithm for various choices of loss functions in Section \ref{sec:Neural_online_learning_regret}.



==> sec/NOR_Regret0.tex <==
In this section we provide regret bounds for online regression using neural networks. We begin with general results under the Polyak-Lojasiewicz (PL) type conditions on the loss function and subsequently obtain regret bounds specifically for squared loss and KL loss. The proof of all the claims have been pushed to Appendix~\ref{sec:Appendix_reg_smooth}. We present our results for the smooth activation architecture here; results for the ReLu architecture can be found in Appendix~\ref{sec:Appendix_reg_relu}.
We begin by introducing the following assumption on the loss function:
\begin{asmp}[{\bf Quadratic Growth (QG)}]
\label{asmp:qg}
The cumulative loss function $\cL(\theta,\z_t) $, $t \in [T]$ satisfy the Quadratic Growth (QG) condition, i.e., there exists a constant $\mu > 0$ such that with $\Theta^*_t = \left\{ \theta_t | \theta_t \in \arg \inf_{\theta} \cL(\theta;\z_t) \right\}, t \in [T]$, for $\theta \in \R^p \setminus \Theta^*_t$, let $\theta^*_t = \Pi_t^*(\theta) \in \Theta^*_t$ be the projection of $\theta$ onto the solution set $\Theta_t^*$, we have 
\begin{align}
    \cL(\theta; \z_t) - \cL(\theta_t^*; \z_t) \geq \frac{\mu}{2} \| \theta - \theta^*_t \|_2^2 ~.
\label{eq:qgcore}
\end{align}
\end{asmp}
\begin{remark}[{\bf QG and PL}]
The recent literature has extensively studied the PL condition and how neural losses satisfy the PL condition~\cite{karimi2016linear, liu2020linearity}. While the Quadratic Growth (QG) condition has not been as widely studied, one can show that the PL condition implies the QG condition~\citep{karimi2016linear}, i.e., for $\mu > 0$
\begin{equation}
\begin{aligned}
  \cL(\theta;\z_t) - \cL(\theta_t^*; \z_t) & \leq \frac{1}{2\mu} \| \nabla \cL(\theta;\z_t) \|_2^2 \quad 
  \Rightarrow \quad   \cL(\theta; \z_t) - \cL(\theta_t^*; \z_t) & \geq \frac{\mu}{2} \| \theta - \theta^*_t \|_2^2   ~.
\end{aligned}
\end{equation}
Thus, the QG condition is more general, and our analysis works with the QG condition.     \qed 
\end{remark}

\begin{algorithm}[t]
\caption{Neural Online Regression}
\begin{algorithmic}[1]
\State Initialize $\theta_1$\;
\For {$t = 1, 2, ..., T$} 
\State Receive an instance $x_t$\;
\State Compute prediction $f(\theta_t; x_t)$  
\State Observe outcome $y_t$\;
\State Update ${\theta}_{t+1} = {\theta}_t - \eta_t \nabla \cL( \theta_t; \z_t )$
\EndFor
\end{algorithmic}
\label{algo:onlineneural}
\end{algorithm}

% Recent work has shown that for neural models with smooth activations, the spectral norm of the Hessian of the predictor can be bounded and shown to decrease with increase in width $m$~\cite{liu2020linearity}. 
Following~\cite{liu2020linearity, liu2022loss} %\abcomment{cite Liu-Zhu-Belkin'20, '21}
, we also assume the following for the activation and loss function: 
\begin{asmp}
For the model in \eqref{eq:DNN_smooth}, the activation $\phi$ is Lipschitz and smooth, i.e., $|\phi'|, |\phi''|$ are bounded; Further, the loss is Lipschitz and strongly convex, i.e., $|\ell_i'|  \leq \lambda, \ell''_i \geq a$ for some constants $\lambda, a > 0$.
\label{asmp:smooth}
\end{asmp}
The Lipschitz loss assumption is not needed for the Hessian spectral norm bound, but it is helpful in simplifying later analysis, and can be relaxed with additional results, e.g., showing that the predictions from \eqref{eq:DNN_smooth} are bounded with high probability (See Lemma~\ref{lemma:lemma_sq_loss_a3} and Lemma~\ref{lemma:lemma_kl_loss_a3}). Then, we have the following result~\citep{liu2020linearity, liu2022loss}.
%\abcomment{cite Liu-Zhu-Belkin'20, '21}
\begin{proposition}[{\bf Hessian Spectral Norm Bound}]
\label{theo:bound-Hess}
Assume the model in \eqref{eq:DNN_smooth} is initialized as $\theta_0$ with $W^{(l)}_{ij} \sim \cN(0,1)$ and $\v$ as a random unit vector. Under Assumption~\ref{asmp:smooth} we have, for any $\x \in \cX$, and
\(
\theta \in B_{\rho}(\theta_0) := \{ \theta | \| \theta - \theta_0 \|_2 \leq \rho \}
\), with a high probability, \rdcomment{refer \cite{banerjee2023restricted}}
\begin{equation}
\label{eq:bound_Hessian}
   \norm{ \nabla^2_\theta f(\theta;\x)}_2 \leq \frac{c_H}{\sqrt{m}}\quad \text{and} \quad \| \nabla_{\theta} f(\theta;\x) \|_2 \leq \varrho~,
\end{equation}
with $c_H = O(\rho^{3L})$ and $\varrho = O(1)$. 
\end{proposition}
%\bancomment{What's the restriction to $\rho$? $\rho \geq 0?$}

% \begin{remark}
% This result shows the spectral norm of the Hessian decreases as the width of the neural network $m$ increases. 
% \end{remark}

The Hessian spectral norm bound can be used to establish the almost (strong) convexity of the loss.

\begin{restatable}[{\bf Almost Strong Convexity of Loss}]{theo}{theoremasc}
Under the conditions of Theorem~\ref{theo:bound-Hess}, with a high probability, \rdcomment{show the dependence on $\delta$ in $\epsilon$?} $\forall \theta' \in  B_{\rho}(\theta_0)$,
\begin{equation}
\label{eq:RSC-formula-NN2}
\begin{aligned}
\hspace*{-5mm} \cL(\theta';\z_t) \geq & \cL(\theta_t;\z_t) + \langle \theta'-\theta_t, \nabla_\theta\cL(\theta_t;\z_t) \rangle
 +  a \left\langle \theta'-\theta_t, \nabla f(\theta'';\z_t) \right\rangle^2 - \epsilon_{t} ~,
\end{aligned}
\end{equation}
where 
\(
\epsilon_{t} = \frac{4 ( 4a \varrho \rho  +  \lambda) c_H \rho^2}{\sqrt{m}}~,
\)
for any $\theta'' \in B_{\rho}(\theta_0)$, where
$c_H$ and $\varrho$ are as in~Theorem~\ref{theo:bound-Hess} and $\lambda, a$ are as in Assumption~\ref{asmp:smooth}. 
\label{theo:rsc2}
\end{restatable}

Different from classical strong convexity, Theorem \ref{theo:rsc2} has an additional term $\epsilon_{t}$ with the order $O(\frac{1}{\sqrt{m}})$. In the limit of $m \rightarrow \infty$, the loss of neural networks exhibits the property of strong convexity. This paves the way for the following regret bound.
\begin{restatable}[\bf Regret Bound under QG condition]{theo}{QGregretsmooth}
\label{thm:PLregret}
Under Assumptions~\ref{asmp:qg} and \ref{asmp:smooth}, if the losses $\cL(\theta,\z_t)$ have unique minimizers, the cumulative loss of Algorithm \ref{algo:onlineneural} with step size $\eta_t = \frac{4}{\mu t}$ satisfies  
\[
\begin{aligned}
    \sum_{t=1}^{T} \cL(\theta_t;\x) - \cL(\theta^*;\x) \leq 2 \sum_{t=1}^T \cL(\theta^\ast, \z_t) + O\left( \log T\right) + O\left(\frac{T}{\sqrt{m}}\right)~,
\end{aligned}
\]

where $\theta^\ast = \arg \min_{\theta \in B_\rho(\theta_0)} \sum_{t=1}^T \cL(\theta, \z_t)$.
\end{restatable}

\rdcomment{Need remarks here}
\rdcomment{Adapt the proof for $n_t$}

Next we show that both squared loss and KL loss for neural models satisfy the assumptions for Theorem \ref{thm:PLregret} under the assumption that the Neural Tangent Kernel (NTK) matrix is positive definite, a mild assumption commonly used in the literature \citep{cao2019generalization,jacot2018neural,du2019gradient,arora2019exact}.
The {\em neural tangent kernel} (NTK) $K_{\ntk}( \cdot,\cdot ; \theta) \in \R^{n \times n}$ corresponding to parameter $\theta$ is defined as 
\(K_{\ntk}(i,j;\theta_t) = \Big\langle\nabla_{\theta}{f}(\theta_t;\x_{t,i}), \nabla_{\theta_T}{f}(\theta;\x_{t,j}) \Big\rangle.\) \rdcomment{Need to change this to NTK at initialization}
\begin{asmp}
    \label{asmp:NTK}
    For all $t\in [0,T]$ we assume that $\lambda_{\min}(K_{\ntk}(\cdot,\cdot;\theta_t)) = \lambda_0 > 0$.
\end{asmp}

\subsection{Regret bounds for Squared Loss}
\label{subsec:sq_loss}
% We consider the squared loss for online regression.
% \begin{align*}
%      {\cL}(\theta;\z_t) = \frac{1}{2} \sum_{i=1}^{n_t} \big({f}(\theta_t;\x_{t,i}) - y_{t,i}\big)^2 
% \end{align*}
The squared loss $\ell_{\sq}(y_{t,i}, \hat{y}_{t,i}) = \frac{1}{2} (y_{t,i} - \hat{y}_{t,i})^2$ for neural models does not have a unique minimizers and therefore one cannot use Theorem~\ref{thm:PLregret}. Towards this, to ensure unique minimizers, we consider an intermediate network with a tiny regularization to the output of the neural network. In detail, given the input $z_t = \{(x_{t,i},y_{t,i})\}_{i=1}^{n_t}$, we consider a network with a tiny regularization as follows:
\begin{align}
\label{eq:output_reg_def}
     \tilde{f}(\theta_t;\x_{t,i}) = f(\theta_t; \x_{t,i}) + c_{\rg}\sum_{j=n_t+1}^{p} \frac{(\theta_t - \theta_0)^Tv_j}{m^{1/4}}
\end{align}
where $\{v_j\}_{j=n_t+1}^{p}$ forms an orthonormal basis that spans the space orthogonal to the subspace spanned by $\{\nabla_{\theta}f(\theta,\x_{t,i})\}_{i=1}^{n_t}$ and $c_{\rg} = 2\lambda c_{H}$.
With slight abuse of notation, we define the cumulative square loss for the original and the regularized respectively as
\begin{align*}
    {{\cL}}_{\sq}(\theta;\z_t) =  \frac{1}{n_t}\sum_{i=1}^{n_t} \ell_{\sq}(y_{t,i},{f}(\theta;\x_{t,i})), \quad  \tilde{{\cL}}_{\sq}(\theta;\z_t) =  \frac{1}{n_t}\sum_{i=1}^{n_t} \ell_{\sq}(y_{t,i},\tilde{f}(\theta;\x_{t,i}))
\end{align*}
The following Lemma shows that the assumptions in Theorem \ref{thm:PLregret} are satisfied for loss function $\tilde{{\cL}}_{\sq}(\theta;\z_t)$ defined above.

\begin{restatable}{lemm}{lemmasqloss}
\label{lemma:lemma_sq_loss_a3}
The following hold for $\theta \in B_{\rho}(\theta_0)$:
\begin{enumerate}
    \item[(i)] With high probability the individual loss function $\ell_{\sq}(y_{t,i},\hat{y}_{t,i})$ is lipschitz and strongly convex with respect to the output $\hat{y}_{t,i}$. \rdcomment{We do not need this here: move to Appendix}
    \item[(ii)] Under Assumption \ref{asmp:NTK} and for width $m > \frac{c_{\rg}^2n_t^2}{\lambda_0^2}$, with high probability the cumulative loss function $\tilde{{\cL}}_{\sq}(\theta;z_t)$ is $\nu$-strongly convex with respect to $\theta$, where $\nu = \mathcal{O}(\frac{1}{\sqrt{m}})$ and satisfies the QG condition with constant $\mu = \lambda_0$.
\end{enumerate}
\end{restatable}
Lemma~\ref{lemma:lemma_sq_loss_a3} along with Theorem~\ref{thm:PLregret} bounds the regret of the regularized network $\tilde{f}(\theta;\x)$. Thereafter we use this to bound the regret of the original network $f(\theta;\x)$ below:
\begin{restatable}[\textbf{Regret Bound for Squared Loss}]{theo}{thmregsq}
    \label{thm:reg_sq_loss_online}
    For the network in \eqref{eq:DNN_smooth}, under assumption \ref{asmp:NTK} and $m = \Omega()$, the regret for Algorithm~\ref{algo:onlineneural} with squared loss $\cL_{\sq}$ can be bounded as:
    \begin{align*}
        R_{\sq}(T) \leq 
    \end{align*}
\end{restatable}
\begin{remark}
    Note that the regularized neural network in \eqref{eq:output_reg_def} is considered for the purposes of analyzing the regret of the original un-regularized network. The core idea of the analysis is to show that the trajectory of the networks are close enough for over parameterized networks and thus one can make use of the regret of the regularized network to bound the regret of the original network. \qed
\end{remark}
\begin{remark}
    The purpose of regularizing the output is to ensure that the corresponding loss is strongly convex and therefore has a unique minimizer. Traditionally this is often achieved by $\ell_2$ -regularization of the loss function. However, it can be shown that although such a regularized loss function is strongly convex, it does not satisfy the PL condition anymore and thus one cannot use Theorem~\ref{thm:PLregret} readily. In constrast, the output regularization considered in \eqref{eq:output_reg_def} ensures that the resulting loss function satisfies both the PL condition and strong convexity. \qed
\end{remark}

\begin{remark}
Since the loss $\tilde{\cL}(\theta;\z)$ is strongly convex, one might wonder why we do not use the standard results from online optimization \citep{} to obtain a $\mathcal{O}(\log T)$ regret directly. This is because the strong convexity constant turns out to be $\nu=\mathcal{O}(1/\sqrt{m})$. Thus, although it is well known that OGD has a regret of $\mathcal{O}(\log T)$ for strongly convex functions, recall that the constant in the order notation scales as $\frac{1}{\nu} = \sqrt{m}$. Thus, the regret will be $O(\sqrt{m} \log T)$. 
To transition from the regret of the regularized to that of the un-regularized loss, observe that in Theorem~\ref{thm:reg_sq_loss_online} 
we need $m=\Omega(T^4)$ and therefore this approach does not yield a $\mathcal{O}(\log T)$ bound. The key idea is to use strong convexity only to ensure a unique minimizer for the loss, while using the PL/QG constant $\mu$ which for neural regression is $\mathcal{O}(1)$ to obtain a $\mathcal{O}(\log T)$ regret.
\qed 
\end{remark}


% \rdcomment{Regret theorem for $\cL_{\sq}$ ?}

% \begin{theorem}
%     Theorem for regret
% \end{theorem}
% The following result bounds the regret in \eqref{eq:online_reg} for squared loss, $R_{\sq}(T)$ and follows from Theorem \ref{thm:PLregret} and Lemma \ref{lemma:lemma_sq_loss_a3}.
% The following result follows from Theorem \ref{thm:PLregret} and Lemma \ref{lemma:lemma_sq_loss_a3}
% \begin{corollary}
%     \label{cor:online_sq_reg}
%     Under Assumption \ref{asmp:NTK}, using Algorithm \ref{algo:onlineneural} with step size $\eta_t = \frac{4}{\mu t}$,
%     \[
%         \begin{aligned}
%            \tilde{\cL}(\theta_t;z_t) - \tilde{\cL}(\theta^*;z_t) \leq 2 \sum_{t=1}^T \cL(\theta^\ast, \z_t) + O\left( \log T\right) + O\left(\frac{T}{\sqrt{m}}\right)~,
%         \end{aligned}
%     \]
% \end{corollary}
\rdcomment{$\theta_t$ remains in the ball?}


\subsection{Regret bounds KL Loss}
\label{subsec:kl_loss}
Next we consider the KL/binary cross-entropy loss defined as follows:
\begin{align*}
 \ell_{\kl}(y_{t,i},\hat{y}_{t,i}) &= -y_{t,i} \ln(\hat{y}_{t,i}) - (1- y_{t,i})\ln(1 - \hat{y}_{t,i}).
\end{align*}
As in Section \ref{subsec:sq_loss}, we consider a regularized network as in \eqref{eq:output_reg_def} and define the cumulative loss for the original and regularized network respectively as:
\begin{align*}
 {\cL}_{\kl}(\theta;\z_t) = \frac{1}{n_t}\sum_{i=1}^{n_t} \ell_{\kl}\big(y_{t,i},\sigma({f}(\theta;\x_{t,i}))\big), \quad \tilde{\cL}_{\kl}(\theta;\z_t) = \frac{1}{n_t}\sum_{i=1}^{n_t} \ell_{\kl}\big(y_{t,i},\sigma(\tilde{f}(\theta;\x_{t,i}))\big).
\end{align*}
Note that here the output of the neural network is passed through a sigmoid which acts as the final output of the network.
As before we show in the next lemma shows that the loss function is strongly convex and satisfies the QG condition.
\begin{restatable}{lemm}{lemmaklloss}
\label{lemma:lemma_kl_loss_a3}
The following hold for $\theta \in B_{\rho}(\theta_0)$:
\begin{enumerate}
    \item[(i)] With high probability the individual loss function $\ell_{\kl}(y_{t,i},\hat{y}_{t,i})$ is lipschitz and strongly convex with respect to the output $\hat{y}_{t,i} = \sigma(\tilde{f}(\theta;\x_{t,i}))$.
    \item[(ii)] Under Assumption~\ref{asmp:NTK} and for $m\geq \frac{C_{\rg}^2n_t^2}{\lambda_0^2q^2(1-q)^2}$, the cumulative loss function ${\cL}_{\kl}(\theta;z_t)$ is (i) strongly convex with respect to the parameters of the model $\theta$ and (ii) satisfies the QG condition with constant $\mu = \lambda_0 q$ where $\forall t$, $\tilde{f}(\theta_t;\z_{t}) \in [q,1-q]$.
\end{enumerate}
\end{restatable}
Lemma~\ref{lemma:lemma_sq_loss_a3} along with Theorem~\ref{thm:PLregret} bounds the regret of the regularized network $\tilde{f}(\theta;\x)$. Thereafter we use this to bound the regret of the original network $f(\theta;\x)$ for KL loss:
\begin{restatable}[\textbf{Regret Bound for KL Loss}]{theo}{thmregsq}
    \label{thm:reg_kl_loss_online}
    For the network in \eqref{eq:DNN_smooth}, under assumption \ref{asmp:NTK} and $m = \Omega()$, the regret for Algorithm~\ref{algo:onlineneural} with KL loss $\cL_{\kl}$ can be bounded as:
    \begin{align*}
        R_{\kl}(T) \leq 
    \end{align*}
\end{restatable}







% \begin{restatable}{lemm}{kllossa3}
% \label{lemma:kl_loss_a3}
%    The individual loss function $\ell_{\kl}(y_{t,i},\hat{y}_{t,i})$ is lipschitz and strongly convex with repect to the output $\hat{y}_{t,i} = \tilde{f}(\theta;\x_{t,i})$ and therefore satisfies Assumption \ref{asmp:smooth}.
% \end{restatable}


% \begin{restatable}{lemm}{kllossscqg}
% \label{lemma:kl_loss_sc_qg}
%    The cumulative loss function ${\cL}_{\kl}(\theta;z_t)$ is $\Theta\left(\frac{1}{\sqrt{m}}\right)$ (i) strongly convex with respect to the parameters of the model $\theta$ and (ii) satisfies the QG condition with constant $\mu = $.
% \end{restatable}


\iffalse







\subsection{Almost (Strong) Convexity of Loss}

Recent work has shown that for neural models with smooth activations, the spectral norm of the Hessian of the predictor can be bounded and shown to decrease with increase in width $m$~\cite{liu2020linearity}. Following~\cite{liu2020linearity, liu2022loss} %\abcomment{cite Liu-Zhu-Belkin'20, '21}
, we start with the following assumption: 
\begin{asmp}
For the model in \eqref{eq:DNN_smooth}, the activation $\phi$ is Lipschitz and smooth, i.e., $|\phi'|, |\phi''|$ are bounded; Further, the loss is Lipschitz and strongly convex, i.e., $|\ell_i'|  \leq \lambda, \ell''_i \geq a$ for some constants $\lambda, a > 0$.
\label{asmp:smooth}
\end{asmp}
The Lipschitz loss assumption is not needed for the Hessian spectral norm bound, is helpful in simplifying later analysis, and can be relaxed with additional results, e.g., showing that the predictions from \eqref{eq:DNN_smooth} are bounded with high probability. Then, we have the following result~\cite{liu2020linearity, liu2022loss}
%\abcomment{cite Liu-Zhu-Belkin'20, '21}
:

\begin{theo}[{\bf Hessian Spectral Norm Bound}]
\label{theo:bound-Hess}
Assume the model in \eqref{eq:DNN_smooth} is initialized as $\theta_0$ with $W^{(l)}_{ij} \sim \cN(0,1)$ and $\v$ as a random unit vector. Under Assumption~\ref{asmp:smooth}, for 
\begin{equation}
\theta \in B_{\rho}(\theta_0) := \{ \theta | \| \theta - \theta_0 \|_2 \leq \rho \}
\end{equation} 
and any $\x$, with high probability,  we have 
\begin{equation}
\label{eq:bound_Hessian}
   \norm{ \nabla^2_\theta f(\theta;\x)}_2 \leq \frac{c_H}{\sqrt{m}}\quad \text{and} \quad \| \nabla_{\theta} f(\theta;\x) \|_2 \leq \varrho~,
\end{equation}
with $c_H = O(\rho^{3L})$ and $\varrho = O(1)$. 
\end{theo}
%\bancomment{What's the restriction to $\rho$? $\rho \geq 0?$}

% \begin{remark}
% This result shows the spectral norm of the Hessian decreases as the width of the neural network $m$ increases. 
% \end{remark}

The Hessian spectral norm bound can be used to establish almost (strong) convexity of the loss.

\begin{restatable}[{\bf Almost (Strong) Convexity of Loss}]{theo}{theorsc}
Under the conditions of Theorem~\ref{theo:bound-Hess}, with high probability, $\forall \theta' \in  B_{\rho}(\theta_0)$,
\begin{equation}
\label{eq:RSC-formula-NN2}
\hspace*{-5mm} \cL(\theta';\z_i) \geq \cL(\theta_t;\z_i) + \langle \theta'-\theta_t, \nabla_\theta\cL(\theta_t;\z_i) \rangle - \epsilon_{t,i} ~,
\end{equation}
where 
\begin{align}
\epsilon_{t,i} = \frac{4 ( 4a \varrho \rho  +  \lambda) c_H \rho^2}{\sqrt{m}} - a \left\langle \theta'-\theta_t, \nabla f(\theta'';\z_i) \right\rangle^2~,
\end{align}
for any $\theta'' \in B_{\rho}(\theta_0)$, where
$c_H$ and $\varrho$ are as in~Theorem~\ref{theo:bound-Hess} and $\lambda, a$ are as in Assumption~\ref{asmp:smooth}. 
\label{theo:rsc2}
\end{restatable}

%\abcomment{need to define $\varrho$, its a poly(L) term with our scaling.}\szcomment{Does $\rho_1$ appear at all in the theorem? Same question for theorem~\ref{theo:bound-Hess}}\szcomment{Is $\ell_{t,i} := \ell(y_i, f(\theta_t, x_i))$? }\szcomment{What is $z_i$? } \abcomment{$\z_i = (\x_i,y_i)$, a data point. The loss $\cL$ depends on $\z_i$, the predictor $f$ only depends on $\x_i$}


\iffalse
\proof For any $\theta' \in B_{\rho}(\theta_0)$, by the second order Taylor expansion around $\theta_t$, we have
\begin{align*}
\cL(\theta';\z_i) & = \cL(\theta_t;\z_i) + \langle \theta' - \theta_t, \nabla_\theta\cL(\theta_t;\z_i) \rangle + \frac{1}{2} (\theta'-\theta_t)^\top \frac{\partial^2 \cL(\tilde{\theta}_t;\z_i)}{\partial \theta^2}
(\theta'-\theta_t)~,
\end{align*}
where $\tilde{\theta}_t = \xi \theta' + (1-\xi) \theta_t$ for some $\xi \in [0,1]$. Since $\theta_t, \theta' \in B_{\rho}(\theta_0)$, we have $\tilde{\theta}_t \in B_{\rho}(\theta_0)$. 

Focusing on the quadratic form in the Taylor expansion, we have
\begin{align*}
(\theta'-\theta_t)^\top \frac{\partial^2 \cL(\tilde{\theta}_t;\z_i)}{\partial \theta^2} (\theta'-\theta_t) 
& = (\theta'-\theta_t)^\top  \left[ \tilde{\ell}''_i \frac{\partial f(\tilde{\theta}_t;\z_i)}{\partial \theta}   \frac{\partial f(\tilde{\theta}_t;\z_i)}{\partial \theta}^\top   + \tilde{\ell}'_i   \frac{\partial^2 f(\tilde{\theta}_t;\z_i)}{\partial \theta^2}      \right] (\theta'-\theta_t) \\
& = \underbrace{\tilde{\ell}''_i \left\langle \theta'-\theta_t, \frac{\partial f(\tilde{\theta}_t;\z_i)}{\partial \theta} \right\rangle^2}_{I_1}    + \underbrace{\tilde{\ell}'_i  (\theta'-\theta_t)^\top \frac{\partial^2 f(\tilde{\theta}_t;\z_i)}{\partial \theta^2}  (\theta'-\theta_t) }_{I_2}~,
\end{align*}
$\tilde{\ell}_i$ corresponds to the loss $\ell(y_i, f_{\tilde{\theta}}(\z_i))$, and $\tilde{\ell}', \tilde{\ell}''_i$ denote the corresponding first and second derivatives w.r.t.~$\hat{\tilde{y}}_i= f_{\tilde{\theta}}(\z_i)$. 

For analyzing $I_1$, choose any $\theta'' \in B_{\rho}(\theta_0)$. Now, note that
\begin{align*}
I_1 & =  \ell''_i \left\langle \theta'-\theta_t, \frac{\partial f(\tilde{\theta}_t;\x_i)}{\partial \theta} \right\rangle^2 \\
& \geq a  \left\langle \theta'-\theta_t, \frac{\partial f(\theta'';\x_i)}{\partial \theta} + \left( \frac{\partial f(\tilde{\theta}_t;\x_i)}{\partial \theta} - \frac{\partial f(\theta'';\x_i)}{\partial \theta} \right) \right\rangle^2 \\
& = a   \left\langle \theta'-\theta_t, \frac{\partial f(\theta'';\x_i)}{\partial \theta} \right\rangle^2 + a  \left\langle  \theta' - \theta_t, \frac{\partial f(\tilde{\theta}_t;\x_i)}{\partial \theta} - \frac{\partial f(\theta'';\x_i)}{\partial \theta} \right\rangle^2 \\
& \qquad \qquad + 2a  \left\langle  \theta' -\theta_t, \frac{\partial f(\theta'';\x_i)}{\partial \theta} \right\rangle  \left\langle  \theta' - \theta_t, \frac{\partial f(\tilde{\theta}_t;\x_i)}{\partial \theta} - \frac{\partial f(\theta'';\x_i)}{\partial \theta} \right\rangle \\
& \geq a \left\langle \theta'-\theta_t, \frac{\partial f(\theta'';\x_i)}{\partial \theta} \right\rangle^2 - 2a \sum_{i=1}^n \left\| \frac{\partial f(\theta'';\x_i)}{\partial \theta} \right\|_2  \left\| \frac{\partial f(\tilde{\theta}_t;\x_i)}{\partial \theta} - \frac{\partial f(\theta'';\x_i)}{\partial \theta} \right\|_2 \| \theta' - \theta_t \|_2 \| \tilde{\theta}_t - \theta''\|_2  \\
& \overset{(a)}{\geq} a  \left\langle \theta'-\theta_t, \nabla f(\theta'';\x_i) \right\rangle^2 - 2a \sum_{i=1}^n \varrho  \frac{c_H}{\sqrt{m}} \| \tilde{\theta}_t - \theta'' \|_2  \| \theta' - \theta_t \|_2 \| \tilde{\theta}_t - \theta''\|_2  \\
& \overset{(b)}{\geq} a \left\langle \theta'-\theta_t, \nabla f(\theta'';\z_i) \right\rangle^2 - \frac{16 a \varrho c_H \rho^3}{\sqrt{m}}~, 
%& \overset{(d)}{\geq} a  \kappa^2 \left\| \frac{\partial f(\theta_t;\x_i)}{\partial \theta} \right\|_2^2 \| \theta' - \theta_t \|_2^2 - \frac{2a \varrho c_H}{\sqrt{m}} \| \theta' - \theta_t \|_2^3  \\
%& \geq \left( a\kappa^2 \left\| \frac{\partial f(\theta_t;\x_i)}{\partial \theta} \right\|_2^2 - \frac{2a\varrho c_H  \| \theta'-\theta_t\|_2}{\sqrt{m}}  \right) \| \theta' - \theta_t \|_2^2 ~,
\end{align*}
where (a) follows from Theorem~\ref{theo:bound-Hess} since $\tilde{\theta_t}\in B_{\rho}(\theta_0)$ and since $\| \nabla f(\theta'';\x_i) \|_2 \leq \varrho$, and (b) follows since $\| \tilde{\theta}_t - \theta'' \|_2, \| \theta' - \theta_t \|_2, \| \tilde{\theta}_t - \theta''\|_2  \leq 2\rho$ by triangle inequality because $\tilde{\theta}, \theta', \theta_t \in B_{\rho}(\theta_0)$.

For analyzing $I_2$,  with $Q_{t,i} = (\theta'-\theta_t)^\top \frac{\partial^2 f(\tilde{\theta}_t;\x_i)}{\partial \theta^2}  (\theta'-\theta_t)$, we have
\begin{align*}
| Q_{t,i} | = \left| (\theta'-\theta_t)^\top \frac{\partial^2 f(\tilde{\theta}_t;\x_i)}{\partial \theta^2}  (\theta'-\theta_t) \right| \leq \| \theta'-\theta_t\|_2^2 \left\| \frac{\partial^2 f(\tilde{\theta}_t;\x_i)}{\partial \theta^2} \right\|_2 \leq \frac{c_H \|\theta' - \theta_t \|_2^2}{\sqrt{m}} \leq \frac{4c_H \rho^2}{\sqrt{m}}~,
\end{align*}
since $\| \theta' - \theta_t \|_2 \leq 2\rho$ by triangle inequality because $\theta', \theta_t \in B_{\rho}(\theta_0)$. Further, since $|\tilde{\ell}_i'| \leq \lambda$ by Assumption~\ref{asmp:smooth}, we have
\begin{align*}
I_2 & =  \tilde{\ell}'_{i}  Q_{t,i} \geq - |\tilde{\ell}'_{i}| | Q_{t,i} | \geq - \frac{4\rho^2 c_H \lambda}{\sqrt{m}}~.
\end{align*}
Putting the lower bounds on $I_1$ and $I_2$ back, we have
\begin{align*}
(\theta'-\theta_t)^\top \frac{\partial^2 \cL(\tilde{\theta}_t)}{\partial \theta^2} (\theta'-\theta_t) 
& \geq a \left\langle \theta'-\theta_t, \nabla f(\theta'';\z_i) \right\rangle^2 - \frac{4 ( 4a \varrho \rho  +  \lambda) c_H \rho^2}{\sqrt{m}}  ~.
\end{align*}
That completes the proof.  \qed 
\fi
\szmargincomment{moved the proof to appendix}




\abcomment{There has to be text earlier (in Section 2 or 3), which establishes what the regret model is, why we will talk about OGD, etc. Otherwise, this abrupt discussion of regret bound from next subsection will not make sense}

%as in~\cite{SD-JL-HL-LW-XZ:19}. 
%but our results can be extended to multi-dimension outputs as in~\cite{DZ-QG:19}, using $\V \in \R^{k \times m_L}$ for $k$ outputs at the last layer.




\subsection{Regret Bound with Polyak-Lojasiewicz (PL) Type Conditions}

% \begin{defn}[PL condition]
% A function $g$ is said to satisfy the PL-condition [][][] if for any $\theta \in \R^p$ and $\theta^*$ denoting an optimum parameter, i.e., $\theta^* \in \arginf_{\theta \in \R^p} g(\theta)$, for some constant $\mu > 0$, we have
% \begin{align}
%     g(\theta) - g(\theta^*) \leq \frac{1}{2\mu} \| \nabla g(\theta) \|_2^2 ~. 
% \label{eq:pldef1}
% \end{align}
% \end{defn}
% % The PL condition can also be written as
% % \begin{align}
% %   g(\theta) - \inf_{\theta' \in \R^d} g(\theta') \leq \frac{1}{2\mu} \| \nabla g(\theta) \|_2^2 ~. 
% % \label{eq:pldef2}
% % \end{align}

% Our regret analysis relies on the relationship between the PL condition and the Quadratic Growth (QG) condition.
% \begin{defn}[QG condition]
% A  function $g$ is said to satisfy the QG-condition [][][] if for any $\theta \in \R^p$ and $\theta^*$ denoting an optimum parameter, i.e., $\theta^* \in \arginf_{\theta \in \R^p} g(\theta)$, for some constant $\mu > 0$, we have
% \begin{align}
%     g(\theta) - g(\theta^*) \geq \frac{\mu}{2} \| \theta - \theta^* \|_2^2 ~. 
% \label{eq:qgdef1}
% \end{align}
% \end{defn}

% \szcomment{$\theta^*$ may be a set (the solution set), so QG and PL is usually defined in terms of projections on to solution set, is that something we need to worry about in the definition / analysis? }

% \abcomment{yes, this is something we will have to worry about --- and this does not look simple ... }



% \begin{lemm}[PL $\Rightarrow$ QG]
% If a function satisfies the PL condition, then it satisfies the QG condition, i.e., for any $\theta \in \R^p$ and $\theta^* \in \arginf_{\theta \in \R^p} g(\theta)$, we have 
% \begin{align}
%  g(\theta) - g(\theta^*) \leq \frac{1}{2\mu} \| \nabla g(\theta) \|_2^2 ~, \forall \theta \not \in \Theta^* \quad \Rightarrow \quad  g(\theta) - g(\theta^*) \geq \frac{\mu}{2} \| \theta - \theta^* \|_2^2 ~, \forall \theta \not \in \Theta^*~.
% \end{align}
% \label{lemm:qgc}
% \end{lemm}
% \abcomment{***unclear*** how to generalize this to a constraint set, e.g., ball around initialization}  

% Next, we focus on cumulative neural losses satisfying the PL condition.
% Consider the cumulative neural loss $g(\theta) = \sum_{t=1}^T \cL(\theta,\z_t)$, and let
% \begin{align}
% \theta^* := \theta^*(\{z_t, t \in [T]\}) \in \underset{\theta \in \R^d}{\arginf}~\sum_{t=1}^T \cL(\theta,\z_t)~.   
% \label{eq:plopt}
% \end{align}
% We denote the set of all such $\theta^*$ as $\Theta^*$. By now, the deep learning literature has extensively studied cumulative neural losses satisfying the PL condition [][][]. In particular, for square loss, if the NTK is positive definite [][], then the cumulative neural loss can be shown to satisfy the PL condition [][]. There is, by now, a sizeable literature on showing the positive definiteness of the NTK [][][].

% \abcomment{ongoing ...}
% \begin{defn}[Neural PL Condition]
% A cumulative neural loss function is said to satisfy the PL-condition [][][] if for any set of $\theta_t \in \R^p, , t \in [T]$ and $\theta^*$ denoting an optimum parameter as in \eqref{eq:plopt}, we have
% \begin{align}
% \forall \theta~, ~~~   \sum_{t=1}^T \cL(\theta_t,\z_t) -  \sum_{t=1}^T \cL(\theta^*,\z_t) \leq \frac{1}{2\mu} \left\| \sum_{t=1}^T \nabla \cL(\theta_t,\z_t) \right\|_2^2 ~. 
% \label{eq:nnpldef1}
% \end{align}
% \end{defn}

% For neural losses, the NTK being positive definite implies the cumulative neural loss satisfies a variant of the PL condition [][][].

In this section, we consider the the regret of an online learner using neural networks under the following assumption.

\begin{asmp}[{\bf Quadratic Growth (QG)}]
%Consider the step-wise neural losses $\cL(\theta_t,\z_t) = \ell(y_t,f_{\theta}(\x_t))$, where $f_{\theta}(\cdot)$ is the neural model. We make the following assumption:
The individual loss functions $\cL(\theta,\z_t) = \ell(y_t,f_{\theta}(\x_t)), t \in [T]$ satisfy the Quadratic Growth (QG) condition, i.e., there exists a constant $\mu > 0$ such that with $\Theta^*_t = \left\{ \theta^*_t | \theta^*_t \in \arg \inf_{\theta} \cL(\theta,\z_t) \right\}, t \in [T]$, for $\theta \in \R^d \setminus \Theta^*_t$, let $\theta^*_t = \Pi_t^*(\theta) \in \Theta^*_t$ be the projection of $\theta$ on to the solution set $\Theta_t^*$, we have 
\begin{equation}
    \cL(\theta, \z_t) - \cL(\theta_t^*, \z_t) \geq \frac{\mu}{2} \| \theta - \theta^*_t \|_2^2 ~.
\label{eq:qgcore}
\end{equation}
\label{asmp:qg}
\end{asmp}
%\szcomment{
%Should be $\cL(\theta, z_t) - \cL(\theta_t^*, z_t) \ge \inf_{\theta_t^*\in \Theta_t^*} \frac{\mu}{2} \norm{\theta - \theta_t^*}^2$? }\abcomment{updated}\szcomment{In defn, the inequality should not hold for all $\theta^*\in \Theta_t^*$, but only the projection of $\theta$ onto $\Theta_t^*$? } \abcomment{good point, I think you are correct, will check; one way to get around this is to assume the arginf is unique; or we may be able to do the proof without additional assumption, but notation has to be updated to capture the projection}\szcomment{I updated the defn, analysis still need to be updated}\abcomment{updated statement, added remark}\szcomment{Thanks, this looks ok}




%
% \szdelete{
% {\bf Interpolation:} The best neural model can interpolate the data $\{(\x_t,y_t)\}$, i.e., for any given $\epsilon > 0$, we can construct a sufficiently over-parameterized neural model $f_{\theta}(\cdot)$ such that
% \begin{equation}
%     \inf_{\theta} \sum_{t=1}^T \cL(\theta,\z_t) =  \inf_{\theta} \sum_{t=1}^T \ell(y_t,f_{\theta}(\x_t)) \leq \epsilon~.
% \label{eq:interpoll}
% \end{equation}
% }
% \szdelete{
% \begin{remark}[Interpolation]
% Recent work in deep learning optimization has extensively established variants of the interpolation condition \abedit{[ALS 2019, Du et al., 2019,  Belkin et al., 18, Noy et al., 2021, Ng et al., 2021]} based on (stochastic) gradient descent applied to the cumulative loss. Typically, the size of the network grows as poly$(T,L)$ and the number of iterations grows as poly$(T,L,\log \frac{1}{\epsilon})$ to bound the cumulative loss with $\epsilon$ as in \eqref{eq:interpoll}. Such existing results usually need a small separation between the inputs, i.e., $\| \x_t - \x_{t'} \|_2 \geq \delta, t \neq t'$, which will translate to restrictions on the adversary. Such results exist both for smooth and ReLU activations \abedit{[ALS 2019, Du et al., 2019]}. \qed 
% \end{remark}
% }

\begin{remark}[{\bf QG and PL}]
The recent literature has extensively studied the PL condition and how neural losses satisfy the PL condition~\cite{karimi2016linear, liu2020linearity}. While the Quadratic Growth (QG) condition has not been as widely studied, one can show that the PL condition implies the QG condition~\cite{karimi2016linear}, i.e., for $\mu > 0$
\begin{equation}
\begin{aligned}
  \cL(\theta, \z_t) - \cL(\theta_t^*, \z_t) & \leq \frac{1}{2\mu} \| \nabla \cL(\theta,\z_t) \|_2^2 \quad \\
  \Rightarrow \quad   \cL(\theta, \z_t) - \cL(\theta_t^*, \z_t) & \geq \frac{\mu}{2} \| \theta - \theta^*_t \|_2^2   ~.
\end{aligned}
\end{equation}
Thus, the QG condition is more general, and our analysis will work with the QG condition.\qed 

\end{remark}

% \begin{defn}[Neural QG Condition]
% A cumulative neural loss function is said to satisfy the QG-condition [][][] if for any set of $\theta_t \in \R^p, t \in [T]$ and $\theta^*$ denoting the optimum parameter as in \eqref{eq:plopt}, we have
% \begin{align}
% \forall \theta~, ~~~ \sum_{t=1}^T \cL(\theta_t,\z_t) -  \sum_{t=1}^T \cL(\theta^*,\z_t)  \geq \frac{\mu}{2} \sum_{t=1}^T \| \theta_t - \theta^* \|_2^2 ~. 
% \label{eq:nnqgcdef1}
% \end{align}
% \end{defn}
% \abcomment{perspective is $g(\theta_1,\ldots,\theta_T)$ with the constraint $\theta_t = \theta_{t'}, t, t' \in [T]$}

% Then, we have the following result:
% \begin{lemm}[Cumulative PL $\Rightarrow$ Cumulative QG]
% If a (loss) satisfies the PL condition, then it satisfies the QGC condition, i.e., 
% \begin{align}
% \sum_{t=1}^T  \cL(\theta_t,\z_t) - \sum_{t=1}^T  \cL(\theta^*,\z_t) & \leq \frac{1}{2\mu} \left\| \sum_{t=1}^T  \nabla \cL(\theta_t,\z_t) \right\|_2^2 ~, \forall \theta \\
% \Rightarrow \quad  \sum_{t=1}^T  \cL(\theta_t,\z_t) - \sum_{t=1}^T \cL(\theta^*,\z_t) & \geq \frac{\mu}{2} \sum_{t=1}^T \| \theta_t - \theta^* \|_2^2 ~, \forall \theta~.
% \end{align}
% \label{lemm:nnqgc}
% \end{lemm}
% \proof \abcomment{... needs a proof ...} \qed
% %\proof The proof follows by a direct application of Lemma~\ref{lemm:qgc} and Definitions~\ref{eq:nnpldef1} and \ref{eq:nnqgcdef1}.\qed 
  
\begin{restatable}[Regret Bound]{theo}{PLregretsmooth}
\label{thm:PLregret}
Under Assumption~\ref{asmp:qg}, \abedit{if the losses $\cL(\theta,\z_t)$ have unique minimizers,} the cumulative loss of $\{ \theta_t, t \in [T]\}$ updated with online gradient descent (OGD) with step size $\eta_t = \frac{4}{\mu t}$ satisfies  
\[
\begin{aligned}
    R(T) &:= \sum_{t=1}^T \cL(\theta_t; \z_t) - \sum_{t=1}^T \cL(\theta',\z_t) \\ 
     &\leq  \sum_{t=1}^T \cL(\theta', \z_t) + O\left( \log T\right) + O\left(\frac{T}{\sqrt{m}}\right)~.
\end{aligned}
\]
for any $\theta' \in B_\rho(\theta_0)$.
\end{restatable}

\begin{remark}
If the losses $\cL(\theta,\z_t)$ do not have unique minimizers, then the result in Theorem~\ref{thm:PLregret} can be extended to get a regret bound with an additional term $\sum_{t=1}^T \| \Pi^*_t(\theta_t) - \Pi^*_t(\theta')\|_2^2$ where $\Pi^*_t(\theta_t), \Pi^*_t(\theta') \in \arginf_{\theta} \cL(\theta,\z_t)$ are respectively the projections of $\theta_t$ and $\theta'$ on the optimal set for $\cL(\theta,\z_t)$. If the optimal set is unique, the term vanishes, yielding Theorem~\ref{thm:PLregret}. \qed 
\end{remark}


%\szcomment{The result seem to imply $\sum_{t} \cL(\theta_t;\z_t) \le O(\log T)$, this seem too good to be true. Consider random labels, the cumulative loss will always be linear, why is this not contradiction? }

%\szcomment{The issue is probably because $\theta^*$ will be outside the desired neighborhood from initialization. }

%\szcomment{One possible fix is to let go of interpolation condition, and replace every $\eps$ in proof by $\sum_t \cL(\theta^*, z_t)$, and final bound we get is $R(T) <= \sum_{t} \cL(\theta^*, z_t) + O(\log T)$. This bound may still be interesting in some cases, say when reward is deterministic and reward function has bounded RKHS norm. Another fix might be to try Massart noise condition ... }

\iffalse
\proof Take any $\tilde{\theta}\in B_\rho(\theta_0)$. By Theorem~\ref{theo:rsc2}, we have
\begin{align*}
    \cL(\theta_t;\z_t) - \cL(\tilde{\theta};\z_t) & \leq \langle \theta_t - \tilde{\theta}, \nabla \cL(\theta_t;\z_t) \rangle + \frac{c_0}{\sqrt{m}}
\end{align*}
where $c_0 = 4 ( 4a \varrho \rho  +  \lambda) c_H \rho^2$. Then,
\begin{align}
\cL(\theta_t;\z_t) - \cL(\tilde{\theta};\z_t) & \leq \langle \theta_t - \tilde{\theta}, \nabla \cL(\theta_t;\z_t) \rangle + \frac{c_0}{\sqrt{m}} \nonumber \\
& = \frac{\langle \theta_t - \tilde{\theta}, \theta_t - \theta_{t+1} \rangle}{\eta_t} + \frac{c_0}{\sqrt{m}}  \nonumber \\
& \leq \frac{ \| \theta_t - \tilde{\theta} \|_2^2 + \|\theta_t - \theta_{t+1}\|_2^2 - \| \theta_{t+1} - \tilde{\theta}\|_2^2 }{2\eta_t} + \frac{c_0}{\sqrt{m}}~ \nonumber \\
& \leq \frac{ \| \theta_t - \tilde{\theta} \|_2^2 - \| \theta_{t+1} - \tilde{\theta}\|_2^2 }{2\eta_t} + \frac{\eta_t}{2} \lambda^2 \varrho^2 + \frac{c_0}{\sqrt{m}}~.
\label{eq:plstep0}
\end{align} 
where we have used $\theta_{t+1} = \theta_t - \eta_t \nabla \cL(\theta_t; \z_t)$, and $\| \theta_t - \theta_{t+1} \|_2 \leq \eta_t \|\nabla_\theta \cL(\theta_t,\x_t) \|_2 \leq \eta_t \lambda \| \nabla_{\theta} f(\theta_t;\x_t)\|_2 \leq \eta_t \lambda \varrho$ from Assumption~\cref{asmp:smooth} \abcomment{Lipschitz loss} and Theorem~\ref{theo:bound-Hess}.


Let $\eta_t = \frac{4}{\mu t}$. Then, summing \eqref{eq:plstep0} over $t=1,\ldots,T$, we have
\bancomment{may want to add the first term here.}
\begin{align}
R(T) &= \sum_{t=1}^T \cL(\theta_t;\z_t)  - \sum_{t=1}^T \cL(\tilde{\theta};\z_t) \nonumber \\
& \leq  \sum_{t=1}^T \| \theta_t - \tilde{\theta}\|_2^2\left( \frac{1}{2\eta_{t}} - \frac{1}{2\eta_{t-1}}   \right) + \frac{\lambda^2 \varrho^2}{2} \sum_{t=1}^T \eta_t  + \frac{c_0 T }{\sqrt{m}} \nonumber \\
& \leq  \frac{\mu}{8} \sum_{t=1}^T \| \theta_t - \tilde{\theta}\|_2^2 + O(\log T) + O\left(\frac{ T }{\sqrt{m}}\right) \nonumber \\
& \leq  \frac{\mu}{4} \sum_{t=1}^T \| \theta_t - \theta_t^*\|_2^2 + \frac{\mu}{4} \sum_{t=1}^T \| \tilde{\theta} - \theta_t^*\|_2^2 + O(\log T) + O\left(\frac{ T }{\sqrt{m}}\right)
\label{eq:plstep1}
\end{align}
where $\tilde{\theta}_t \in \arginf_{\theta} \cL(\theta; \z_t)$.  



%\bancomment{In the second line, why don't just let $\eta_t = \eta_{t-1}$? Such that the first term will be zero.} \abcomment{we have a $\sum_t \eta_t$ term, keeping $\eta_t$ constant will make this term $T$.} \bancomment{With this choice of $\eta_t$, can we show that the trajectories of $\theta$ will still stay in the ball? }
%\bancomment{I am a little skeptical to the choice of $\eta$. In the Cao-Gu's paper, the choice of $\eta$ is to reduce $\frac{\| \theta_1 - \theta^\ast \|^2_2}{\eta}$ and $\frac{\lambda^2 \varrho^2}{2} \sum_{t=1}^T \eta_t$ at the same time while keeping $\theta$ in the ball. In contrast, we choose different $\eta_t$ at different rounds to remove the above two terms. But how can we guarantee $\theta$ will still stay in the ball? }

% \abdelete{Multiplying \eqref{eq:plstep2} by $-1/2$ adding to \eqref{eq:plstep1}, we have
% \begin{align}
% -\frac{1}{2}\left(\sum_{t=1}^T \cL(\theta_t;\z_t) - \sum_{t=1}^T \cL(\theta^*;\z_t)\right) & \leq - \frac{\mu}{2} \sum_{t=1}^T  \| \theta_t - \theta^* \|_2^2~.
% \label{eq:plstep2}
% \end{align}
% \szcomment{The first term should be $\sum_{t=1}^T \sum_{t'=1}^T \cL(\theta_t; z_{t'})$ if we are using PL on the loss function $\sum_{t=1}^T \cL(\theta; z_t)$} \abcomment{updated the notation, this may be resolved now, i'll check}\szcomment{The cumulative loss function is $\sum_{t=1}^T \cL(\theta^*; z_t)$, so a PL gives $\sum_{t=1}^T \cL(\theta;z_t) - \sum_{t=1}^T \cL(\theta^*; z_t) > \mu \norm{\theta - \theta^*}_2^2$, this in no way translates to $\sum_{t=1}^T \cL(\theta_t;z_t) - \sum_{t=1}^T \cL(\theta^*; z_t) > \mu \sum_{t=1}^T \norm{\theta_t - \theta^*}_2^2$, since we cannot be plugging in a different $\theta_t$ in summand in first term or rhs. }
%Adding \eqref{eq:plstep1} and \eqref{eq:plstep2}, and multiplying both sides by 2, we get}
% \begin{align}
% \sum_{t=1}^T & \cL(\theta_t;\z_t)  - \sum_{t=1}^T \cL(\theta^*;\z_t) \\
% & \leq   2 \sum_{t=1}^T \| \theta_t - \theta^*\|_2^2\left( \frac{1}{\eta_{t}} - \frac{1}{\eta_{t-1}} - \frac{\mu}{2}  \right) + 2 \sum_{t=1}^T \| \theta^* - \theta_t^*\|_2^2\left( \frac{1}{\eta_{t}} - \frac{1}{\eta_{t-1}}   \right) + 2 \lambda^2 \varrho^2 \sum_{t=1}^T \eta_t  + \frac{2 c_0 T }{\sqrt{m}}~,
% \end{align}

By Assumption~\ref{asmp:qg}, the neural losses satisfy the QG condition, so that for $t \in [T]$
\begin{align}
\cL(\theta_t,\z_t) - \cL(\theta_t^*,\z_t) & \geq \frac{\mu}{2} \| \theta_t - \theta_t^* \|_2^2~, \label{eq:plstep2a} \\
\cL(\theta^*,\z_t) - \cL(\theta_t^*,\z_t) & \geq \frac{\mu}{2} \| \theta^* - \theta_t^* \|_2^2~. \label{eq:plstep2b}
\end{align}

\szdelete{
Further, by Assumption~\ref{asmp:qg}, since the interpolation condition is satisfied, we have
\begin{align}
\sum_{t=1}^T \cL(\theta^*,\z_t) - \sum_{t=1}^T \cL(\theta_t^*,\z_t) \leq \sum_{t=1}^T \cL(\theta^*,\z_t) \leq \epsilon~,
\label{eq:plstep3}
\end{align}
\bancomment{Where is the definition of $\theta^\ast$?   Compared to $\theta^\ast_t$}\abcomment{will add, $\theta^* = \sum_{t=1}^T \cL(\theta;\z_t)$, so this is the best model using all the data, this satisfied the interpolation condition}
for any suitably chosen constant $\epsilon > 0$. 
}

Then, we can lower bound the regret as
\begin{align}
R(T) &= \sum_{t=1}^T \cL(\theta_t;\z_t)  - \sum_{t=1}^T \cL(\theta^*;\z_t) \nonumber \\
& = \sum_{t=1}^T \left(\cL(\theta_t;\z_t) - \cL(\theta_t^*,\z_t)\right)  - \sum_{t=1}^T (\cL(\theta^*;\z_t) - \cL(\theta_t^*,\z_t)) \nonumber \\
& \geq \frac{\mu}{2} \sum_{t=1}^T \| \theta_t - \theta_t^* \|_2^2 - \szedit{\sum_{t=1}^T \cL(\theta^*; \z_t)} ~,
\label{eq:plstep4}
\end{align}
from \eqref{eq:plstep2a}\szdelete{and \eqref{eq:plstep3}}. Multiplying \eqref{eq:plstep4} by $-\frac{1}{2}$ and adding to \eqref{eq:plstep1}, we get
\begin{align*}
\frac{1}{2} R(T) & = \sum_{t=1}^T \cL(\theta_t;\z_t)  - \sum_{t=1}^T \cL(\theta^*;\z_t) \\
& \leq \frac{\mu}{4} \sum_{t=1}^T \| \theta^* - \theta_t^*\|_2^2 + O(\log T) + O\left(\frac{ T }{\sqrt{m}}\right) + \frac{\szedit{\sum_{t=1}^T \cL(\theta^*; \z_t) }}{2} \nonumber \\
& \overset{(a)}{\leq} \frac{1}{2} \sum_{t=1}^T ( \cL(\theta^*,\z_t) - \cL(\theta_t^*,\z_t) ) + O(\log T) + O\left(\frac{ T }{\sqrt{m}}\right) + \frac{\szedit{\sum_{t=1}^T \cL(\theta^*; \z_t) }}{2} \nonumber \\
& \overset{(b)}{\leq} \szedit{\sum_{t=1}^T \cL(\theta^*; \z_t) } + O(\log T) + O\left(\frac{ T }{\sqrt{m}}\right) \nonumber \\
& = O(\szedit{\sum_{t=1}^T \cL(\theta^*; \z_t) } + \log T) + O\left(\frac{ T }{\sqrt{m}}\right)~,
\end{align*}
That completes the proof. \qed 
\fi
\szmargincomment{moved to appendix}





% \abcomment{makes things precise} \szcomment{What is $\theta^*$, global optimum or optimum for $z_t$? If $\theta^*$ is global optimum, then the line after $\cref{eq:plstep1}$ will not hold. In general we won't have $L(\theta_t, z_t) - L(\theta^* , z_t) > \mu \norm{\theta_t - \theta^*}_2^2 / 2$. } \abcomment{if the cumulative loss satisfies PL, then would imply QG on the cumulative loss; there is existing work which shows that cumulative square loss satisfies PL for neural models if the NTK is positive definite}

% \abcomment{main technical challenge: how to extend this to the setting where PL is satisfied within a ball around initialization? many associated questions: (1) PL need not imply invexity in a ball, (2) gradient flow may leave the ball}

% \bancomment{To make sure that the gradient flow won't leave the ball, we may need  $\mu_t \geq  \sqrt{m}$}.

\subsection{Regret bound for ReLU architecture}

Recall that $B_{\rho}(\theta_0) := \{ \theta | \| \theta - \theta_0 \|_2 \leq \rho\}$.
%Recall that $ \B(\theta_0, \omega) = \{\theta: \|\theta - \theta_0\|_2 \leq \omega\}$.\hecomment{This has been defined in the previous section with $B_{\rho}(\theta_0)$.} 
We have the following results.

\iffalse
\begin{defn}
Let $\Theta_T = \{ \theta_t, t \in [T]\}$ be the parameter trajectory of online gradient descent.
For some $\kappa \in (0,1]$, define
\begin{equation}
\hspace*{-3mm}
    S_{\kappa}(\B(\theta_0, \omega), \Theta_T) := \bigg\{ \theta \in \B(\theta_0, \omega) ~\bigg|~ \forall t \in [T], ~ \exists \theta_t'' \in \B(\theta_0, \omega) ~\text{s.t}~ |\cos(\theta - \theta_t, \nabla f(\theta_t'';\x_t)) | \geq \kappa \bigg\}~.
\end{equation}
\end{defn}
\fi



\begin{lemma} [Almost Strong Convexity] \label{lemma:relursc}
Suppose the loss function $\mathcal{L}$ satisfies the strong convexity.
With probability at least $1 - \delta$ over the randomness of $\theta_0$, for any $\theta' \in B_{\rho}(\theta_0)$, we have 
\begin{equation} 
\begin{aligned}
\cL(\theta'; \z_t)  \ge & \cL(\theta_t; \z_t) +    \ip{\nabla_\theta \cL(f(\theta))}{\theta' - \theta_t}  \\
& +  \ip{\nabla f(x_i; \theta_t)}{\theta'-\theta_t}^2  - \epsilon_{R}.
\end{aligned}
\end{equation}
where $ \epsilon_{R} = \big [ O(\rho^{4/3}L^2 \sqrt{m\log m})  +  O(\rho^{7/3}  L^2 m \sqrt{\log m} )  \big ]$
\end{lemma}


\begin{theorem} [Regret Bound]
Under Assumption~\ref{asmp:qg}, if the losses $\cL(\theta,\z_t)$ have unique minimizers,
with probability at least $1- \delta$ over the randomness of initialization, for any $R \geq 0$, with $\omega \leq \frac{R}{\sqrt{m}}$, $m \geq O( T^2 R^2 L^{12} (\log m)^{4/3} )$ , and $\eta_t =  m \kappa^2 \sum_{\tau =1}^{t-1}\| \nabla f (\theta_\tau; \mathbf{z}_\tau) \|_2^2$ , the cumulative loss for online gradient descent after $T$ rounds is 
\begin{equation}
\sum_{t=1}^T \cL(\theta_t;\z_t)  \leq  2 \sum_{t=1}^T  \cL(\theta^*;\z_t) + O(\log T)  + O(\frac{TR}{m^{1/6}}).
\end{equation}
\end{theorem}


\begin{remark}
The regret bound of ReLU network is comparable to smooth network, but with a different error term $O(\frac{TR}{m^{1/6}}).$ This is because ReLU activation function does not possess the property of Lipschitz smooth, while it has a semi-smoothness property when $m$ is wide enough \cite{allen2019convergence}. Thus, we need a wider network to diminish the term to $O(1)$, achieving the $\log T$ online regret bound.    
\end{remark}









\fi
